Poles, Residues and Siegel-Weil Identities of Degenerate Eisenstein Series on Split Exceptional Groups of Type $E_n$

This manuscript has two goals: 1. To write an explicit description of the degenerate residual spectrum of the split, simple, simply-connected, exceptional groups of type $E_n$ (for $n=6,7,8$). 2. To set a practical guide for similar calculations and, in particular, to describe various methods of ``computational representation theory'' relevant to the study of residues of automorphic Eisenstein series. In Part I we supply background information and notations from the theory of automorphic representations as well as concrete information on the exceptional groups of type $E_n$ and their representation theory over non-Archimedean local fields. In Part II we make a systematic study of the residual spectrum of these groups where each chapter is devoted to a certain aspect of theory, it begins with methodical section and continues with sections devoted to the results for each of these groups. We describe completely the residual (square-integrable and non-square integrable) spectrum of the groups of type $E_6$ and $E_7$ and an almost complete description in the case of the group of type $E_8$. We also study and list Siegel-Weil like identities between residual representations of these groups and list the Arthur parameters for their square-integrable residual representations.

==> poles_with_tables_instead_of_longtables.tex <==
\chapter{Poles of Degenerate Eisenstein Series}
\label{Chap:Poles_of_Eisen_ser}


In this part, we study the poles of the degenerate Eisenstein series.
That is, we describe the set of poles of $\Eisen_{P_i} \bk{f,s,\chi,g}$ and determine the order of these poles.


\section{The Method}
\label{Section:Poles_Method}

\subsection{The Constant Term at a Point and Equivalence Classes}

Let $f_s=\otimes_{v\in\Places} f_{s,v}$ be a factorizable standard section and assume that $f_{s,v}=f_{s,v}^0$ for $v\notin S$, where $S\subset\Places$ is a finite set of primes of $F$.

It follow from \Cref{Eq:Constant_term} and \Cref{Eq:Global_GK_Formula} that
\begin{equation}
	\label{eq::CT_first_form}
	\begin{split}
		\Eisen_{P_i} \bk{f,s,\chi,g}_T 
		& = \suml_{w\in W^{M,T}} M_w\bk{\lambda_{s,\chi}^{P_i}} f_s\bk{g} \\
		& = \suml_{w\in W^{M,T}} C_w\bk{\lambda_{s,\chi}^{P_i}} \otimes_{v\notin S}f_{s,v}\bk{g_v} \otimes_{v\in S} N_{w,v}\bk{\lambda_{s,\chi}^{P_i}}f_{s,v}\bk{g_v} \\
	\end{split}
\end{equation}
Each summand may have a pole of a certain order and, by summation, the orders of these poles can be reduced, that is different summands may cancel each others poles.

We consider the constant term $\Eisen_{P_i} \bk{f,s,\chi,g}_T$ as a representation of $T$; as such, each summand on the right-hand-side of \Cref{eq::CT_first_form} lies within a single isotypic component.
Thus, cancellations of poles may happen only within the same isotypic component.
Thus, given $\chi$ and $s_0\in\C$, we define an equivalence relation $\sim_{s_0,\chi}$ on $W^{M,T}$ as follows:
\[
w\sim_{s_0,\chi}w' \Leftrightarrow w\cdot\lambda_{s_0} = w'\cdot\lambda_{s_0} .
\]
Thus, we may rewrite \Cref{eq::CT_first_form} by summing over equivalence classes as follows
\begin{equation}
	\label{eq::CT_second_form}
	\Eisen_{P_i} \bk{f,s,\chi,g}_T = 
	\suml_{\coset{w'}\in W^{M,T}\rmod\sim_{s_0,\chi}}  \kappa_{\coset{w'}}\bk{f,g},
\end{equation}
where
\begin{equation}
	\label{eq::sum_over_eq_cl}
	\begin{split}
		\kappa_{\coset{w'}}\bk{f,s,g} 
		& = \suml_{w\in\coset{w'}} M_w\bk{\lambda_{s,\chi}^{P_i}} f_s\bk{g} \\
		& = \suml_{w\in\coset{w'}} C_w\bk{\lambda_{s,\chi}^{P_i}} \otimes_{v\notin S}f_{s,v}\bk{g_v} \otimes_{v\in S} N_{w,v}\bk{\lambda_{s,\chi}^{P_i}}f_{s,v}\bk{g_v} .
	\end{split}
\end{equation}

We note that the poles of each summand can arise either from the Gindikin-Karpelevich factor $C_w\bk{\lambda_{s,\chi}^{P}}$ or from the local intertwining operators $N_{w,v}\bk{\lambda_{s,\chi}^{P}}f_{s,v}\bk{g_v}$.
We will show that, for $\Real\bk{s}>0$, the local factors do not contribute to the order.
That is, the order of the pole of each summand is determined by the order of $C_w\bk{\lambda_{s,\chi}^{P}}$.

We also point out that the order of $M_w\bk{s,\chi}$ is constant on an equivalence class $\coset{w'}$.
We write $\equivclassespole{s_0,\chi,k}$ for the set of equivalence classes in $W^{M,T}\rmod\sim_{s_0,\chi}$ which satisfy:
\[
\ord{s=s_0}{M_w\bk{s,\chi}} \geq k \quad \forall w\in\coset{w'} .
\]
We say that a pole of order $k$ of $\Eisen_{P_i} \bk{f,s,\chi,g}$ is canceled or reduced, if $\equivclassespole{i,s_0,\chi,k}\neq \emptyset$, while $\ord{s=s_0}{\Eisen_{P_i} \bk{f,s,\chi,g}}<k$.



\subsection{Holomorphicity of Local Normalized Intertwining Operators}

In our analysis of the poles of degenerate Eisenstein series and their residues, we make use of the following property of local intertwining operators:

\hbox{}
\textbf{\underline{Property A:}}
The operator $N_{w,v}\bk{\lambda}$ is well-defined and holomorphic at $\lambda_{s,\chi}^{P_i}$ for all $w\in W^{M_i,T}$ and $s\in\C$ such that $\Real\bk{s}>0$.
\hbox{}\\

It is known that \textbf{Property A} holds due to \cite{Zhang1997,Arthur1989,MR581582,Kostant1978,Vogan1978,Muic2001,MR1341660}.
%[Zhang Yunali, The holomorphy and non-vanishing of ..., Theorem 3]
%[Arthur, Intertwining operators and residues..., \S 3]
%[Casselman-Shalika, The unramified principal..., 1980]
%[Kostant, On Whittaker vectors..., 1978]
%[Vogan, Gelfand-Kirillov dimension..., 1978]
%[Muic, A proof of Casselman-Shahidh conjecture..., 2001]
%[Jantzen, On Iwahori-Matsumuto involution..., 1995, ]

\begin{comment}
	Bellow, we explain how to prove \textbf{Property A} for $G=E_6$.
	In the case of $G=E_7$ and $G=E_8$, the proof works for the absolute majority of quintuples $\bk{i,s_0,\chi,w,v}$.
	However, there were a number of such quadruples for which the methods described bellow was not enough to prove \textbf{Property A}.
	For most of these cases $\chi$ is trivial and thus, the validation of \textbf{Property A} can be reduced to a calculation performed in the context of the Iwahori-Hecke algebra.
	The relevant operators can be realized as acting on the space of Iwahori-fixed vectors $\DPS{P_i}\bk{s_0,\chi}_v^{\mathcal{J}_v}$ and holomorphicity can be checked this way.
	For an explanation on how to realize these operators in Sagemath, see \cite[Appendix B]{SDPS_E7}.
	However, this would require lengthy computing time and thus, we work under the following assumption:
	
	\begin{Conj}
		\textbf{Property A} holds for $G$ of type $E_7$ and $E_8$.
	\end{Conj}
	
	\begin{proof}[Proof of Property A for $G=E_6$]
		Fix a place $v\in\Places$.
		We separate the proof to a number of cases:
		
		The simplest case is when $\chi$ is unramified and $\DPS{{P_i}}\bk{s,\chi}$ is generated by its spherical vectors.
		In this case, it holds that 
		\begin{equation}
			\label{eq::normalized_intertwining_operator_on_spherical_vector}
			N_{w,v}f_{\lambda_{s,\chi}^{P_i},v}^0 = f_{w\cdot\lambda_{s,\chi}^{P_i},v}^0 .
		\end{equation}
		Assume that $N_{w,v}f_{\lambda_{s,\chi}^{{P_i}},v}\bk{g}$ admits a pole at $s_0$ for some section $f_{\lambda_{s,\chi}^{P}}\in \DPS{{P_i}}\bk{s,\chi}$ and $g\in G_v$.
		Then, the residue of $N_{w,v}f_{\lambda_{s,\chi}^{P_i},v}$ at $s_0$ generates a quotient of $\DPS{{P_i}}\bk{s_0,\chi}$.
		It follows that $N_{w,v}f_{\lambda_{s,\chi}^{P_i},v}^0$ also admits a pole, contradicting \Cref{eq::normalized_intertwining_operator_on_spherical_vector}.
		
		We now consider the proof for ramified $\chi$ or in the case that $\DPS{P}\bk{s,\chi}$ is not generated by the spherical vector.
		
		By \cite{MR517138} and \cite{MR563369}, the partially normalized operator
		\[
		\bk{\prodl_{\alpha\in R\bk{w}} \Lfun_v\bk{\inner{\lambda,\check{\alpha}}}}^{-1} M_{w,v}\bk{\lambda}
		\]
		is entire and non-vanishing.
		Hence, the normalized intertwining operator $N_{w,v}\bk{\lambda}$ admits a pole at $\lambda_{s_0,\chi}^{P}$ only if
		\[
		\Lambda_{w,v}\bk{\lambda} = \prodl_{\alpha\in R\bk{w}} \Lfun_v\bk{\inner{\lambda,\check{\alpha}}+1}
		\]
		does.
		For most triples $\bk{s_0,\chi,w}$, with $\Real\bk{s_0}>0$, the product $\Lambda_{w,v}\bk{\lambda}$ is holomorphic at $\lambda_{s_0}$.
		However, for a quadruple $\bk{i,s_0,\chi,w}$ such that $\Lambda_{w,v}\bk{\lambda}$ is not holomorphic at $\lambda_{s_0}$, one can still prove that $N_{w,v}\bk{\lambda}$ is, using the following argument.
		
		
		Let $w'$ denote the shortest element in $\coset{w}\in W^{M,T}\rmod\sim_{s_0,\chi}$ and write
		\[
		w=\bk{u_r\cdots u_1}w' ,
		\]
		where for each $1\leq j\leq r$, one of the following holds:
		\begin{itemize}
			\item The function $\Lambda_{u_j,v}\bk{u_{j-1}\cdots u_1w_0\cdot\lambda}$ is holomorphic at $\lambda_{s_0,\chi}^{P}$, and hence the operators $N_{u_j}\bk{u_{j-1}\cdots u_1w_0\cdot\lambda}$ is holomorphic there too.
			\item The element $u_j=w_{i_1}\cdots w_{i_k}$ satisfies the following properties:
			\begin{itemize}
				\item $u_j\in\Stab_W\bk{u_{j-1}\cdots u_1w_0\cdot\lambda}$.
				\item $i_1=i_k$.
				\item $i_t\neq i_1$ for any $1<t<k$.
				\item $\inner{u_{j-1}\cdots u_1w_0,\check{\alpha_{i_1}}}=\pm1$.
				\item $\inner{\s{i_1}u_{j-1}\cdots u_1w_0,\check{\alpha_{i_t}}}=0$ for any $1<t<k$.
			\end{itemize}
			In these circumstances, it follows from \Cref{Prop:Zampera} that the operator
			\[
			N_{u_j}\bk{u_{j-1}\cdots u_1w_0\cdot\lambda}\res{\lambda_{s,\chi}^{P_i}}
			\]
			is well-defined and holomorphic at $s_0$.
			
		\end{itemize}
		
		
	\end{proof}
\end{comment}



\begin{Cor}
	\begin{enumerate}
		\item The order of $M_w\bk{\lambda_{s,\chi}^{P_i}} f_s\bk{g}$ at $s_0$ equals that of $C_w\bk{\lambda_{s,\chi}^{P_i}}$.
		\item If $\Eisen_{P_i} \bk{f,s,\chi,g}$ admits a pole at $s_0\in\C$, with $\Real\bk{s_0}>0$, then there exists $w\in W^{M,T}$ such that $C_w\bk{\lambda_{s,\chi}^{P_i}}$ admits a pole at $s_0$.
		
		
	\end{enumerate}
\end{Cor}

Thus, in order to find all of the poles of $\Eisen_{P_i} \bk{f,s,\chi,g}$ with $\Real\bk{s_0}>0$, one can proceed with the following steps:

\begin{enumerate}
	\item Find all $\chi$, $s_0$ and $w\in W^{M,T}$ such that $C_w\bk{\lambda_{s,\chi}^{P_i}}$ admits a pole at $s_0$.
	
	\item Bound the order of $\Eisen_{P_i} \bk{f,s,\chi,g}$ from above by $n$.
	We use two methods to perform this step:
	\begin{enumerate}
		\item For $\chi$ and $s_0$ and $w$ as above, determine the order of $\kappa_{\coset{w}}$ and let $n$ be the maximum of the orders of such poles using a reduction of orders of poles, as described in \Cref{Subsection:Methods_Reduction_of_order_of_poles}.
		
		\item In case that $\chi$ is trivial and $\DPS{P}\bk{s_0}$ is generated by its spherical vector (i.e. $\DPS{P}\bk{s_0}$ admits a unique irreducible quotient), we follow \cite{MR1174424} and use a method described in \Cref{Subsection:Poles_Method_Normalized_Eis_ser}.
	\end{enumerate}
	
	\item Prove that some equivalence class $\coset{w'}\in W^{M,T}\rmod\sim_{s_0,\chi}$ realizes a pole of order $n$.
	That is, show that
	\[
	\ord{s=s_0}{\kappa_{\coset{w'}}} = n .
	\]
	Usually, this can be done using a singleton $\set{w}\in W^{M,T}\rmod\sim_{s_0,\chi}$ such that the order of $C_w\bk{\lambda_{s,\chi}^{P}}$ at $s_0$ is $n$.
	
	\item Finally, we wish to determine the square-integrability of the residual representation.
	We do this using Langlands' criterion as detailed in \Cref{Subsection:Square-Integrability_criterion}.
\end{enumerate}

\begin{Rem}
	\label{Rem:Order_of_trivial_eq_class}
	We point out that $\set{1}\in W^{M,T}\rmod\sim_{s_0,\chi}$ for any $\Real\bk{s_0}>0$ and that $\ord{s=s_0}{\kappa_{\set{1}}}=0$.
	Hence, for any $\Real\bk{s_0}>0$, we have $\ord{s=s_0}{\Eisen_{P_i}\bk{\chi}}\geq 0$.
\end{Rem}




\subsection{Reduction of Orders of Poles}
\label{Subsection:Methods_Reduction_of_order_of_poles}

Considering the sum $\kappa_{\coset{w'}}\bk{f,s,g}$ in \Cref{eq::sum_over_eq_cl}, it is possible that each summand $M_w\bk{\lambda_{s,\chi}^{P_i}} f_s\bk{g}$ admits a pole of order $n$, yet $\kappa_{\coset{w'}}\bk{f,s,g}$ itself will admit a pole of a lower order or even be holomorphic.

The main reason for the cancellation of these poles is as follows.
Assume that $w'$ is the shortest element in $\coset{w'}$ and let $\lambda=w'\cdot\lambda_{s_0,\chi}^{P_i}$.

We note that the coset $\coset{w'}$ can be written as follows
\[
\coset{w'} = \set{uw' \mvert u\in \Stab_W\bk{\lambda} \cap \bk{W^{M,T} \cdot \bk{w'}^{-1}} } 
\]
We assume that $\Stab_W\bk{\lambda} \cap \bk{W^{M,T} \cdot \bk{w'}^{-1}}$ is isomorphic to $\bk{\bZ\rmod2\bZ}^k$, or in other words, it can be written as
\begin{equation}
	\label{Eq:Equivalence_class_as_a_shifted_product_of_Z/2Z}
	\coset{w'} = \set{uw' \mvert u \in \prodl_{i=1}^k \set{1,u_i} }.
\end{equation}


Finally, we assume that
\begin{equation}
	\label{Eq:Global_interwining_operator_acts_as_-1}
	M_{u_i}\bk{\lambda} \varphi = -\varphi \qquad \forall\varphi\in \Res{s=s_0} \coset{M_{w}\bk{\lambda_{s,\chi}^{P_i}}\bk{\DPS{P_i}\bk{s,\chi}}} .
\end{equation}
For $\varphi\in \Res{s=s_0} \coset{M_{w}\bk{\lambda_{s,\chi}^{P_i}}\bk{\DPS{P_i}\bk{s,\chi}}}$, it holds that
\[
\prodl_{i=1}^k \bk{\Id+M_{u_i}\bk{\lambda}}\varphi \in o\bk{\bk{s-s_0}^k} .
\]

It follows that
\[
\max\set{\ord{s=s_0}{M_w\bk{s,\chi}}} = n \quad \Rightarrow \quad \ord{s=s_0}{\kappa_{\coset{w'}}\bk{f,s,g}} \leq n-k .
\]

We list bellow a couple methods of validating \Cref{Eq:Global_interwining_operator_acts_as_-1}:
\begin{enumerate}
	\item Assume that $u_i$ can be written as $u_i=u_0^{-1}\cdot z\cdot u_0$, where $N_{u_0}\bk{\lambda}$ is an isomorphism and $z=s_{j_1}\cdot...\cdot s_{j_l}$, where
	\[
	\inner{u_0\cdot\lambda,\check{\alpha_{j_1}}} = ... = \inner{u_0\cdot\lambda,\check{\alpha_{j_l}}} = 0 .
	\]
	Then, by \cite[Proposition 6.3]{MR944102},
	\[
	M_z\bk{u_0\cdot\lambda} = \bk{-1}^l Id .
	\]
	If $l$ is odd, it follows that
	\[
	\begin{split}
		M_{u_i}\bk{\lambda} 
		& = M_{u_0^{-1}}\bk{z\cdot u_0 \cdot\lambda} \circ N_z\bk{u_0\cdot\lambda} \circ M_{u_0}\bk{\lambda} \\
		& =	- M_{u_0^{-1}}\bk{u_0 \cdot\lambda} \circ Id \circ M_{u_0}\bk{\lambda} \\
		& =	- M_{u_0^{-1}}\bk{u_0 \cdot\lambda} \circ M_{u_0}\bk{\lambda} = -Id .
	\end{split}
	\]
	
	\item Assume that $u_i$ can be written as $u_i=u_0^{-1}\cdot z\cdot u_0$, where $M_{u_0}\bk{\lambda}$ is an isomorphism and that $M_z\bk{u\cdot\lambda}$ satisfies the conditions of \Cref{Prop:Zampera}.
	Then, $N_z\bk{u\cdot\lambda}_v$ is holomorphic and diagonalizable at $s=s_0$ for all $v\in\Places$.
	Further assume that
	\[
	C_z\bk{u\cdot\lambda} \underset{s\to s_0}{\longrightarrow} -1 
	\]
	and that $N_{u_0w',v}\bk{\lambda_{s_0,\chi}}\bk{\DPS{P}\bk{s_0,\chi}_v}$ is contained within the $1$-eigenspace of $N_z\bk{u_0\cdot\lambda}$.
	Then,
	\[
	M_z\bk{u_0\cdot\lambda}=-Id.
	\]
	One concludes that $M_{u_i}\bk{\lambda}=-Id$ as in the previous item.
	
	We now explain how, given $v\in\Places_{fin.}$, to check that $N_{u_0w',v}\bk{\lambda_{s_0,\chi}^{P_i}}\bk{\DPS{P_i}\bk{s_0,\chi}_v}$ is, indeed, contained within the $1$-eigenspace of $N_z\bk{u_0\cdot\lambda_{s_0,\chi}^{P_i}}$, under the assumption that $\pi_v=\DPS{P_i}\bk{s_0,\chi}_v$ admits a unique irreducible quotient $\pi_{1,v}$.
	
	Let $\lambda_{0,v}$ denote the initial exponent of $\pi_v$ and let $\lambda_1=u_0w'\cdot\lambda_0$.
	We write $z=s_j z' s_j$, where $\inner{\lambda_{1},\check{\alpha_j}}=\pm 1$.
	By \Cref{Prop:Zampera}, $i_T^G\lambda_1$ decomposes as follows
	\[
	i_{T_v}^{G_v}\lambda_1 = \underbrace{i_{L_{j,v}}^{G_v}\bk{\tau_{tr.}}}_{1-eigenspace} \oplus \underbrace{i_{L_{j,v}}^{G_v}\bk{\tau_{St.}}}_{\epsilon-eigenspace},
	\]
	where $\tau$ is a $1$-dimensional representation of $L_{j,v}$, $\epsilon<0$ and
	\[
	\tau_{tr.}=\tau\otimes \Id_{L_{j,v}},\quad 
	\tau_{St.}=\tau\otimes \St_{L_{j,v}} .
	\]
	Now, since $N_{u_0w'}\bk{\pi}$ is a quotient of $\pi$, it also admits a unique irreducible quotient.
	It follows that $N_{u_0w'}\bk{\pi} \subset i_{L_{j,v}}^{G_v}\bk{\tau_{tr.}}$ or $N_{uw'}\bk{\pi} \subset i_{L_{j,v}}^{G_v}\bk{\tau_{St.}}$.
	It thus remains to prove that $N_{u_0w'}\bk{\pi} \subset i_{L_{j,v}}^{G_v}\bk{\tau_{tr.}}$, this would follow from the following calculation (if true):
	\begin{itemize}
		\item $s_j\cdot\lambda_1\leq r_T^G\bk{i_{L_{j,v}}^{G_v}\bk{\tau_{tr.}}}$.
		\item $s_j\cdot\lambda_1\nleq r_T^G\bk{i_{L_{j,v}}^{G_v}\bk{\tau_{St.}}}$.
		\item $s_j\cdot\lambda_1\leq r_T^G\pi_{1,v}$.
	\end{itemize}
	While the first two items follow from \Cref{Prop:Zampera}, the third follows from a branching rule calculation (see \Cref{Appendix:Branching_Rules} for more details).
\end{enumerate}

\begin{Rem}
	In some cases, we use a variation of the above method.
	Namely, we replace \Cref{Eq:Equivalence_class_as_a_shifted_product_of_Z/2Z} with the assumption that
	\[
	\coset{w'} \cdot \bk{w'}^{-1} \subseteq \prodl_{i=1}^k \set{1,u_i}
	\]
	and that for any $u\in \prodl_{i=1}^k \set{1,u_i}$ such that $uw'\notin W^{M,T}$, it holds that $M_{uw}$ vanishes on the degenerate principal series $\DPS{P_i}\bk{s,\chi}$ to the $l^{th}$ order.
	Hence, for any $f_s\in \DPS{P}\bk{s,\chi}$ it holds that
	\[
	\suml_{w\in\coset{w'}} M_{w}f_s = \suml_{u\in \prodl_{i=1}^k \set{1,u_i}} M_{uw'}f_s
	\]
	Under these assumptions, it is possible to apply the above methods on the right-hand-side instead of the left one, taking the order $l$ of the zeros of the added intertwining operators into account.
\end{Rem}

\vbox{}

We would also like to mention a slightly more complex variation of the application of \Cref{Prop:Zampera} mentioned above.
We consider the following situation:
\begin{itemize}
	\item Fix $v\in\Places_{fin.}$, we assume that $\pi_v$ admits a unique irreducible quotient $\pi_{1,v}$.
	\item $\lambda=w'\cdot\lambda_{s_0,\chi}^{P_i}$.
	\item $\coset{w'} = \set{w',u w'}$.
	\item The Weyl element $u$ can be written in the form $u=u_0^{-1}\cdot z\cdot u_0$, where $N_{u_0}\bk{\lambda_{s_0,\chi}^{P_i}}$ is an isomorphism such that $\lambda_1=u_0\cdot\lambda$ and $z$ satisfy the following conditions:
	\begin{itemize}
		\item $z\in W_L$, where $L=L_\Theta$, $\Theta\subset\Delta$, is a standard Levi subgroup of $G$ of type $A_5$.
		\item Furthermore, denote the elements of $\Theta$ by $\alpha_{j_1},...,\alpha_{j_5}$ such that the sub-Dynkin diagram of $\Delta$ induced by $\Theta$ is
		\[\begin{tikzpicture}[scale=0.5]
			\draw (-1,0) node[anchor=east]{};
			\draw (0 cm,0) -- (8 cm,0);
			\draw[fill=black] (0 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_{j_1}$};
			\draw[fill=black] (2 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_{j_2}$};
			\draw[fill=black] (4 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_{j_3}$};
			\draw[fill=black] (6 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_{j_4}$};
			\draw[fill=black] (8 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_{j_5}$};
		\end{tikzpicture}\]
		\item $z=w_{j_2}w_{j_4}tw_{j_2}w_{j_4}$, where $t\in\gen{w_{j_1},w_{j_3},w_{j_5}}$.
		\item The restriction $\mu$ of $\lambda_1$ to $L$, under the isomorphism with the $A_5$ root system, written with respect to the basis of fundamental weights, is given by
		\[
		\mu=\bk{-1,1,-1,1,-1} .
		\]
	\end{itemize}
\end{itemize}

In this case, we argue that, $N_{uw',v}\bk{\lambda_{s_0,\chi}^{P_i}}\bk{\DPS{P_i}\bk{s_0,\chi}_v}$ is contained within the $1$-eigenspace of $N_z\bk{u\cdot\lambda}$ and hence one may continue as above.

Indeed, by \cite[Example 5.5]{SegalSingularities}, the representation $i_{T_v}^{G_v}\lambda_1$ decomposes into a direct sum of the $\pm1$-eigenspaces of $N_{w_{j_2}w_{j_1}w_{j_2}}$ and $N_{w_{j_4}w_{j_5}w_{j_4}}$ respectively.
Namely,
\[
i_{T_v}^{G_v}\lambda_1 = \oplus_{\delta,\epsilon\in\set{-1,1}} \pi_{\delta,\epsilon},
\]
where $\pi_{\delta,\epsilon}$ is the $\delta$-eigenspace of $N_{w_{j_2}w_{j_1}w_{j_2}}$ and the $\epsilon$-eigenspace of $N_{w_{j_4}w_{j_5}w_{j_4}}$.

Write $\lambda_2=w_{j_4}w_{j_2}\cdot \lambda_1$, this is an anti-dominant exponent when restricted to $L$ and it appears with full multiplicity in $\pi_{1,1}$.
One may conclude that $N_z\bk{\lambda_1}$ acts on $\pi_{1,1}$ as $\Id$.

Thus, if $\lambda_2$ is an exponent of $\pi_{1,v}$, we may conclude that it is the image $N_{u_0w'}\bk{\lambda_{s_0,\chi}\bk{\pi}^{P_i}}$ and it is a subrepresentation of $\pi_{1,1}$ and hence $N_{u}\bk{\lambda}$ acts on it as $\Id$.


\begin{Rem}
	Similar arguments can be made for $L_\Theta$ of type $A_6$ and $D_6$, all of which have been considered in \cite[Section 5.2]{SegalSingularities}.
\end{Rem}

%A slightly more peculiar application of \Cref{Prop:Zampera} and \cite[Corollary 5.1]{SegalSingularities} was not portrayed in \cite{SegalSingularities} and we wish to set it here.
%We assume the following setting:
%\begin{itemize}
%	\item Fix $v\in\Places_{fin.}$, we assume that $\pi_v$ admits a unique irreducible quotient $\pi_{1,v}$.
%	\item Let $\lambda=w'\cdot\lambda_{s_0,\chi}^{P_i}$ and assume that $\coset{w'} = \set{w',u w'}$.
%	\item The Weyl element $u$ can be written in the form $u=u_0^{-1}\cdot z\cdot u_0$, where $N_{u_0}\bk{\lambda_{s_0,\chi}^{P_i}}$ is an isomorphism such that $\lambda_1=u_0\cdot\lambda$ and $z$ satisfy the following conditions:
%	\begin{itemize}
	%		\item $z\in W_L$, where $L=L_\Theta$, $\Theta\subset\Delta$, is a standard Levi subgroup of $G$ of type $A_3$.
	%		\item Denote the elements of $\Theta$ by $\alpha_{j_1},\alpha_{j_2},\alpha_{j_3}$ so that the sub-Dynkin diagram of $\Delta$ induced by $\Theta$ is
	%		\[\begin{tikzpicture}[scale=0.5]
		%			\draw (-1,0) node[anchor=east]{};
		%			\draw (0 cm,0) -- (4 cm,0);
		%			\draw[fill=black] (0 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_{j_1}$};
		%			\draw[fill=black] (2 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_{j_2}$};
		%			\draw[fill=black] (4 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_{j_3}$};
		%		\end{tikzpicture}\]
	%		\item $z=w_{j_1} w_{j_2} w_{j_1} w_{j_3} w_{j_2} w_{j_3} = w_{j_2} w_{j_1} w_{j_3} w_{j_2}$.
	%		\item The restriction $\mu$ of $\lambda_1$ to $L$, under the isomorphism with the $A_3$ root system, written with respect to the basis of fundamental weights, is given by
	%		\[
	%		\mu=\bk{1,-1,1} .
	%		\]
	%	\end{itemize}
%\end{itemize}
%
%In this situation, the Weyl elements $z_1=w_{j_1} w_{j_2} w_{j_1}$ and $z_3=w_{j_3} w_{j_2} w_{j_3}$ would each satisfy the conditions of \Cref{Prop:Zampera}.
%This brings about a decomposition
%\[
%i_{T_v}^{G_v}\lambda_1 = \oplus_{\delta,\epsilon\in\set{-1,1}} \pi_{\delta,\epsilon},
%\]
%where $\pi_{\delta,\epsilon}$ is the $\delta$-eigenspace of $N_{z_1}\bk{\lambda_1}$ and the $\epsilon$-eigenspace of $N_{z_3}\bk{\lambda_1}$.
%We point out that $i_{T_v}^{L_v}\lambda_1$ is of length $4$ so all of the $\pi_{\delta,\epsilon}$ are distinct non-zero subspaces of $i_{T_v}^{G_v}\lambda_1$.
%Finally, we wish to point out that $z_1$ and $z_3$ are commuting elements in $W_L$ and hence \cite[Corollary 5.1]{SegalSingularities} applies.
%One proceeds as in the previous case.






\subsection{Bounds on the Order of the Pole for trivial $\chi$}
\label{Subsection:Poles_Method_Normalized_Eis_ser}

Here we note an alternative method for bounding the order of $\Eisen_{P_i} \bk{f,s,\chi,g}$ in the case that $\chi=\Id$.

We recall that the spherical normalized Eisenstein series,
\[
\Eisen_{B}^\sharp\bk{\lambda,g} = 
\coset{\prodl_{\alpha\in\Phi^+} \zfun\bk{l_\alpha^+\bk{\lambda}} l_\alpha^+\bk{\lambda} l_\alpha^-\bk{\lambda}}
\Eisen_{B}\bk{f^0_\lambda,\lambda,g} ,
\]
given in \Cref{qq:Normalized_Eisenstein_Series}, is entire and $W_G$-invariant.
Following \cite{MR1174424}, we consider the value of $\Eisen_{B}^\sharp\bk{\eta_s^{P_i},g}$.


\begin{Prop}
	It holds that
	\[
	\Eisen_{B}^\sharp\bk{w\cdot \eta_s^{P_i},g} = G_{P_i}\bk{s} \cdot \Eisen_{P_i}^{G} \bk{f^0,s,\chi,g},
	\]
	where $G_{P_i}\bk{s}$ is holomorphic on $\Real\bk{s}>0$.
	In particular, with $\Real\bk{s_0}$, the order of the pole of $\Eisen_{P_i}^{G} \bk{f^0,s,\chi,g}$ at $s_0$ is bounded from above by the order of the zero of $G_{P_i}\bk{s}$ at $s_0$.
\end{Prop}

\begin{proof}
	This follows from \Cref{Prop:Equality_of_Eisenstein_series}, the term $G_{P_i}\bk{s}$ is given by the elements of the normalizing factor other than thus associated with the hyperplanes $\frakh_k$.
\end{proof}

In particular, at points $s_0$ where $\Real\bk{s_0}>0$ and $\DPS{P_i}\bk{s_0}$ is generated by the spherical vector (i.e., it admits a unique irreducible quotient), it holds that $\Eisen_{P_i}^{G} \bk{f,s,\chi,g}$ admits a pole only if $\Eisen_{P_i}^{G} \bk{f^0,s,\chi,g}$ does.
Furthermore, if $\Eisen_{P_i}^{G} \bk{f^0,s,\chi,g}$ admits a pole, then $G_{P_i}\bk{s_0}=0$.
Thus, under these assumptions, the set of poles of $\Eisen_{P_i}^{G} \bk{f,s,\chi,g}$ in $\Real\bk{s_0}>0$ is contained by the set of zeros of $G_{P_i}\bk{s}$ there.
Let
\[
N_\epsilon\bk{\lambda} = \set{\alpha\in\Phi^{+} \mvert \inner{\lambda,\check{\alpha}}=\epsilon}
\]
and let $d_{P_i}\bk{s_0}$ denote the order of the zero of $G_{P_i}\bk{s}$ at $s_0$.
The following proposition determines the value of $d_{P_i}\bk{\eta_s}$ when $F=\Q$ and $s\in\R$.
The assumption that $F=\Q$ is made only so that the denominator of the Gindikin-Karpelevich factors is non-vanishing for $\Real\bk{s}>0$.

\begin{Prop}
	If $F=\Q$ and $s\in\R$, then
	\[
	d_{P_i}\bk{\lambda_s^{P_i}} = \Card{N_1\bk{\lambda_s^{P_i}}}-\Card{N_0\bk{\lambda_s^{P_i}}}-\bk{n-1} .
	\]
\end{Prop}

\begin{proof}
	Since $\Delta_M\subseteq N_1\bk{\lambda_s^{P_i}}$, it follows that
	\[
	\begin{split}
		G_{P_i}\bk{s} = & \bk{\prodl_{\alpha\in N_{-1} \bk{\lambda_s^{P_i}}} \zfun\bk{l_\alpha^+\bk{\lambda}} l_\alpha^+\bk{\lambda} l_\alpha^-\bk{\lambda}} \\
		& \times \bk{\prodl_{\alpha\in N_{0} \bk{\lambda_s^{P_i}}} \zfun\bk{l_\alpha^+\bk{\lambda}} l_\alpha^+\bk{\lambda} l_\alpha^-\bk{\lambda}} \\
		& \times \bk{\prodl_{\alpha\in N_{1} \bk{\lambda_s^{P_i}} \setminus \Delta_M } \zfun\bk{l_\alpha^+\bk{\lambda}} l_\alpha^+\bk{\lambda} l_\alpha^-\bk{\lambda}} \\
		& \times \bk{\prodl_{\alpha\in \Phi^{+} \setminus N_{1,0,-1} \bk{\lambda_s^{P_i}}} \zfun\bk{l_\alpha^+\bk{\lambda}} l_\alpha^+\bk{\lambda} l_\alpha^-\bk{\lambda}} ,
	\end{split}
	\]
	where
	\[
	N_{\epsilon_1,...,\epsilon_l}\bk{\lambda} = \bigcup_{i=1}^l N_{\epsilon_i}\bk{\lambda} .
	\]
	On the other hand, it holds that
	\[
	\begin{split}
		& \prodl_{\alpha\in N_{0} \bk{\lambda_s^{P_i}}} l_\alpha^+\bk{\lambda} l_\alpha^-\bk{\lambda} = \bk{-1}^{\Card{N_{0} \bk{\lambda_s^{P_i}}}} \\
		& \prodl_{\alpha\in N_{1} \bk{\lambda_s^{P_i}} \setminus \Delta_M } l_\alpha^+\bk{\lambda} l_\alpha^-\bk{\lambda} = \coset{2\zfun\bk{2}}^{ \Card{N_{0} \bk{\lambda_s^{P_i}}} -\bk{n-1}} \\
		& \prodl_{\alpha\in N_{-1} \bk{\lambda_s^{P_i}}} l_\alpha^-\bk{\lambda} = \bk{-2}^{\Card{N_{-1} \bk{\lambda_s^{P_i}}}} .
	\end{split}
	\]
	Note, in particular, that $\Card{\Delta_M}=n-1$.
	
	Hence,
	\[
	\begin{split}
		G_{P_i}\bk{s} = & \bk{\prodl_{\alpha\in N_{-1} \bk{\lambda_s^{P_i}}} \zfun\bk{l_\alpha^+\bk{\lambda}} l_\alpha^+\bk{\lambda}} \times \bk{\prodl_{\alpha\in N_{0} \bk{\lambda_s^{P_i}}} \zfun\bk{l_\alpha^+\bk{\lambda}} } \\
		& \times \bk{\prodl_{\alpha\in N_{1} \bk{\lambda_s^{P_i}} \setminus \Delta_M } \zfun\bk{l_\alpha^+\bk{\lambda}} } \times \bk{\prodl_{\alpha\in \Phi^{+} \setminus N_{1,0,-1} \bk{\lambda_s^{P_i}}} \zfun\bk{l_\alpha^+\bk{\lambda}} l_\alpha^+\bk{\lambda} l_\alpha^-\bk{\lambda} } \\
		& \times 
		\zfun\bk{2}^{ \Card{N_{0} \bk{\lambda_s^{P_i}}} -\bk{n-1}} \times
		\bk{-1}^{\Card{N_{0,-1} \bk{\lambda_s^{P_i}}}} \times
		2^{\Card{N_{1,-1} \bk{\lambda_s^{P_i}}} -\bk{n-1} } .
	\end{split}
	\]
	Under our assumptions, it turns out the the following terms are holomorphic and non-zero
	\[
	\begin{split}
		& \prodl_{\alpha\in N_{-1} \bk{\lambda_s^{P_i}}} \zfun\bk{l_\alpha^+\bk{\lambda}} l_\alpha^+\bk{\lambda} , \\
		& \prodl_{\alpha\in \Phi^{+} \setminus N_{1,0,-1} \bk{\lambda_s^{P_i}}} \zfun\bk{l_\alpha^+\bk{\lambda}} l_\alpha^+\bk{\lambda} l_\alpha^-\bk{\lambda}, \\
		& \zfun\bk{2}^{ \Card{N_{0} \bk{\lambda_s^{P_i}}} -\bk{n-1}} \times
		\bk{-1}^{\Card{N_{0,-1} \bk{\lambda_s^{P_i}}}} \times
		2^{\Card{N_{1,-1} \bk{\lambda_s^{P_i}}} -\bk{n-1} } .
	\end{split}
	\]
	Hence, the order of the zero of $G_{P_i}\bk{s}$ at $s=s_0$ is that of
	\[
	\bk{\prodl_{\alpha\in N_{0} \bk{\lambda_s^{P_i}}} \zfun\bk{l_\alpha^+\bk{\lambda}} } \times \bk{\prodl_{\alpha\in N_{1} \bk{\lambda_s^{P_i}} \setminus \Delta_M } \zfun\bk{l_\alpha^+\bk{\lambda}} }
	\]
	and hence
	\[
	d_{P_i}\bk{\lambda_s^{P_i}} = \Card{N_1\bk{\lambda_s^{P_i}}}-\Card{N_0\bk{\lambda_s^{P_i}}} - \bk{n-1} .
	\]
\end{proof}

In particular, it follows that:
\begin{Cor}
	Under the same assumptions, there exist a non-zero constant $C\in\C^\times$ such that 
	\[
	\Eisen_{B}^\sharp\bk{\lambda_{s_0}^{P_i},g} = C \cdot \Res{s=s_0} \Eisen_{P_i} \bk{f_{\lambda_s^{P_i}}^0,s,\Id,g} .
	\]
\end{Cor}

We conclude this discussion be formulating a test for the existence and order of a pole.
For a point $s_0$ such that $C_w\bk{\lambda_{s,\chi}^{P_i}}$ admits a pole at $s_0$ for some $w\in W^{M,T}$, $\DPS{P_i}\bk{s_0}$ is generated by its spherical vector and $d_{P_i}\bk{\lambda_s}>0$, one expects that the order of $\Eisen_{P_i}^{G} \bk{f,s,\chi,g}$ at $s_0$ equals $d_{P_i}\bk{\lambda_s}>0$.
This can usually be verified by finding a singleton $\set{w}\in W^{M,T}\rmod\sim_{s_0,\chi}$ such that the order of $\ord{s_0}{C_w\bk{\lambda_{s,\chi}^{P_i}}}=d_{P_i}\bk{\lambda_s}$.



\subsection{Square-Integrability of the Residue}
\label{Subsection:Square-Integrability_criterion}

In order to determine whether the residual representation $\Res{s=s_0} \Eisen_{P}\bk{\chi}$ is square-integrable, that is admits an embedding into $L^2\bk{Z_\AA G_F\lmod G_\AA,\chi}$, we will use the Langlands' square-integrability criterion \cite[page 104]{MR0579181}.
Assume that $\Eisen_{P}\bk{\chi}$ admits a pole of order $k$ at $s=s_0$ and let
\[
\Sigma^{\bP,0}_{\bk{s_0,\chi,m}} = 
\set{ \coset{w'} \in \Sigma^{\bP}_{\bk{s_0,\chi,m}} \mvert
	\lim\limits_{s\to s_0} \bk{s-s_0}^k \kappa_{\coset{w'}}\bk{f,s,g} \not\equiv 0}
\]
\begin{Prop}[Langlands' Square-integrability Criterion]
	\label{Prop:Square_integrability_of_residue}
	The residual representation $\Res{s=s_0} \Eisen_{P}\bk{\chi}$ is square-integrable if and only if $\Real\bk{w'\cdot \lambda_{s_0,\chi}^{P}}<0$ for all $\coset{w'}\in \Sigma^{\bP,0}_{\bk{s_0,\chi,m}}$.
\end{Prop}


\section{Results for $E_6$}

\begin{Thm}
	The orders of poles of the degenerate Eisenstein series $\Eisen_{P_i}^{G} \bk{f,s,\chi,g}$ are given in the tables bellow.
	The tables also state whether the residue is square-integrable or not.
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_1$, $P_6$ & $3$ & $6$ \\ \hline
			\multirow{2}{*}{1} & Pole Order & 1 & 1 \\ 
			& $L^2$ & $\cmark$ & $\cmark$ \\ \hline
		\end{tabular}
	\end{table}
	
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_2$ & $\frac{1}{2}$ & $\frac{5}{2}$ & $\frac{7}{2}$ & $\frac{11}{2}$ \\ \hline
			\multirow{2}{*}{1} & Pole Order & 1 & 1 & 1 & 1 \\ 
			& $L^2$ & $\cmark$ & $\xmark$ & $\cmark$ & $\cmark$ \\ \hline
			\multirow{2}{*}{2} & Pole Order & 1 & 0 & 0 & 0 \\ 
			& $L^2$ & $\cmark$ &  &  &  \\ \hline
		\end{tabular}
	\end{table}
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_3$, $P_5$ & $\frac{3}{2}$ & $\frac{5}{2}$ & $\frac{7}{2}$ & $\frac{9}{2}$ \\ \hline
			\multirow{2}{*}{1} & Pole Order & 2 & 1 & 1 & 1 \\ 
			& $L^2$ & $\cmark$ & $\xmark$ & $\xmark$ & $\cmark$ \\ \hline
			\multirow{2}{*}{2} & Pole Order & 1 & 0 & 0 & 0 \\ 
			& $L^2$ & $\cmark$ &  &  &  \\ \hline
		\end{tabular}
	\end{table}
	
	
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_4$ & $\frac{1}{2}$ & $1$ & $\frac{3}{2}$ & $\frac{5}{2}$ & $\frac{7}{2}$ \\ \hline
			\multirow{2}{*}{1} & Pole Order & 2 & 1 & 3 & 2 & 1 \\ 
			& $L^2$ & $\xmark$ & $\xmark$ & $\cmark$ & $\cmark$ & $\cmark$ \\ \hline
			\multirow{2}{*}{2} & Pole Order & 1 & 1 & 1 & 0 & 0 \\ 
			& $L^2$ & $\xmark$ & $\xmark$ & $\cmark$  & &  \\ \hline
			\multirow{2}{*}{3} & Pole Order & 1 & 0 & 0 & 0 & 0 \\ 
			& $L^2$ & $\cmark$ &  &  & &  \\ \hline
		\end{tabular}
	\end{table}
	
\end{Thm}


\begin{proof}
	We start by noting the symmetry between the cases $i=1$ and $i=6$ and between $i=3$ and $i=5$.
	Thus, we only consider the cases $1\leq i\leq 4$.
	
	In each case $\bk{P_i,s_0,ord\bk{\chi}}$, we calculate the maximal order of pole of any particular intertwining operator.
	Namely,
	\begin{equation}
		\label{Eq:E6_highest_int_op_pole_order}
		\max\set{ord\bk{M_w\bk{s,\chi}} \mvert w\in W^{M,T}}
	\end{equation}
	These are given in the following tables:
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_1$, $P_6$ & $1$ & $2$ & $3$ & $4$ & $5$ & $6$ \\ \hline
			1 & Pole Order & 2 & 2 & 2 & 1 & 1 & 1 \\ \hline
		\end{tabular}
	\end{table}
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_2$ & $\frac{1}{2}$ & $\frac{3}{2}$ & $\frac{5}{2}$ & $\frac{7}{2}$ & $\frac{9}{2}$ & $\frac{11}{2}$ \\ \hline
			1 & Pole Order & 4 & 3 & 3 & 2 & 1 & 1 \\ \hline
			2 & Pole Order & 1 & 0 & 0 & 0 & 0 & 0 \\ \hline
		\end{tabular}
	\end{table}
	
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_3$, $P_5$ & $\frac{1}{2}$ & $1$ & $\frac{3}{2}$ & $\frac{5}{2}$ & $\frac{7}{2}$ & $\frac{9}{2}$ \\ \hline
			1 & Pole Order & 5 & 1 & 5 & 3 & 2 & 1 \\ \hline
			2 & Pole Order & 1 & 1 & 1 & 0 & 0 & 0 \\ \hline
		\end{tabular}
	\end{table}
	
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_4$ & $\frac{1}{6}$ & $\frac{1}{2}$ & $1$ & $\frac{3}{2}$ & $\frac{5}{2}$ & $\frac{7}{2}$ \\ \hline
			1 & Pole Order & 1 & 9 & 2 & 6 & 3 & 1 \\ \hline
			2 & Pole Order & 0 & 3 & 2 & 1 & 0 & 0 \\ \hline
			3 & Pole Order & 1 & 1 & 0 & 0 & 0 & 0 \\ \hline
		\end{tabular}
	\end{table}
	
	In the case of trivial $\chi$, the order of the Eisenstein series $\Eisen_{P_i}^{G} \bk{f,s,\chi,g}$ is bounded by the orders given in the statement of the theorem using the method described in \Cref{Subsection:Poles_Method_Normalized_Eis_ser}.
	On the other hand, these orders are realized by a singleton $\set{w}\in W^{M,T}\rmod\sim_{s_0,\chi}$ such that the order of $C_w\bk{\lambda_{s,\chi}^{P_i}}$ at $s_0$ is as required.
	
	We now consider the case of non-trivial $\chi$.
	There are a couple of distinct cases that should be taken cared of here:
	\begin{enumerate}
		\item If the order given by \Cref{Eq:E6_highest_int_op_pole_order} equals that of the statement of the theorem, it is enough to provide an equivalence class $\coset{w'}\in W^{M,T}\rmod\sim_{s_0,\chi}$ which realizes a pole of this order.
		The relevant cases are: $\bk{2, 1/2, 2}$, $\bk{3, 3/2, 2}$ and $\bk{4, 3/2, 2}$.
		
		In the case $\bk{4,1/2,3}$, there is no singleton equivalence class which supports a pole.
		However, in \Cref{Chap:Square_Integrable} we calculate the residue of the $\kappa_{\coset{w'}}\bk{f,s,g}$ which support a simple pole.
		In particular, the Eisenstein series admits a simple pole there.
		
		\item If the order given by \Cref{Eq:E6_highest_int_op_pole_order} is lower than that in the statement of the theorem, then one uses the method described in \Cref{Subsection:Methods_Reduction_of_order_of_poles}, in order to provide a lower bound to $\ord{s=s_0}{\Eisen_{P_i}^{G} \bk{f,s,\chi,g}}$ which would agree with the order stated in the theorem.
		There are, then, two cases:
		\begin{enumerate}
			\item If $\ord{s=s_0}{\Eisen_{P_i}^{G} \bk{f,s,\chi,g}} = 0$, then $\Eisen_{P_i}^{G} \bk{f,s,\chi,g}$ is holomorphic.
			Consider \Cref{Rem:Order_of_trivial_eq_class} to see that it is also non-vanishing.
			The relevant cases are: $\bk{3, 1/2, 2}$, $\bk{3, 1, 2}$ and $\bk{4, 1/6, 3}$.
			These are also the cases where $\DPS{P_i}\bk{s_0,\chi}_v$ is irreducible for any $v\in\Places$.
			
			\item Otherwise, there exists a singleton equivalence class which supports a pole of the prescribed order, as in item (1).
			The relevant cases are $\bk{4, 1/2, 2}$ and $\bk{4, 1, 2}$.
		\end{enumerate}
		
		
	\end{enumerate}
	
	In order to determine the square-integrability of the residue, we employ \Cref{Prop:Square_integrability_of_residue}.
	
\end{proof}


\section{Results for $E_7$}

\begin{Thm}
	The orders of poles of the degenerate Eisenstein series $\Eisen_{P_i}^{G} \bk{f,s,\chi,g}$ are given in the tables bellow.
	The tables also state whether the residue is square-integrable or not.
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_1$& $\frac{1}{2}$ & $\frac{7}{2}$ & $\frac{11}{2}$ & $\frac{17}{2}$ \\ \hline
			\multirow{2}{*}{1} & Pole Order & 1 & 1 & 1 & 1 \\ 
			& $L^2$ & $\cmark$ & $\cmark$ & $\cmark$ & $\cmark$ \\ \hline
			\multirow{2}{*}{2} & Pole Order & 1 & 0 & 0 & 0 \\ 
			& $L^2$ & $\cmark$ &  &  &  \\ \hline
		\end{tabular}
	\end{table}
	
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_2$& $1$ & $2$ & $3$ & $4$ & $5$ & $7$ \\ \hline
			\multirow{2}{*}{1} & Pole Order & 1 & 1 & 1 & 1 & 1 & 1 \\ 
			& $L^2$ & $\cmark$ & $\xmark$ & $\xmark$ & $\xmark$ & $\cmark$ & $\cmark$  \\ \hline
			\multirow{2}{*}{2} & Pole Order & 0 & 1 & 0 & 0 & 0 & 0 \\ 
			& $L^2$ &  & $\cmark$ &&&&  \\ \hline
		\end{tabular}
	\end{table}
	
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_3$& $\frac{1}{2}$ & $\frac{3}{2}$ & $\frac{5}{2}$ & $\frac{7}{2}$ & $\frac{9}{2}$ & $\frac{11}{2}$ \\ \hline
			\multirow{2}{*}{1} & Pole Order & 2 & 2 & 2 & 1 & 1 & 1 \\ 
			& $L^2$ & $\cmark$ & $\cmark$ & $\cmark$ & $\xmark$ & $\xmark$ & $\cmark$ \\ \hline
			\multirow{2}{*}{2} & Pole Order & 1 & 1 & 1 & 0 & 0 & 0 \\ 
			& $L^2$ & $\cmark$ & $\cmark$ & $\cmark$ &  &  &  \\ \hline
			\multirow{2}{*}{3} & Pole Order & 1 & 0 & 0 & 0 & 0 & 0 \\ 
			& $L^2$ & $\cmark$ &  &  &  &  &  \\ \hline
		\end{tabular}
	\end{table}
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_4$& $\frac{1}{2}$ & $\frac{2}{3}$ & $1$ & $\frac{3}{2}$ & $2$ & $3$ & $4$ \\ \hline
			\multirow{2}{*}{1} & Pole Order & 1 & 1 & 4 & 1 & 3 & 2 & 1 \\ 
			& $L^2$ & $\xmark$ & $\xmark$ & $\cmark$ & $\xmark$ & $\cmark$ & $\cmark$ & $\cmark$  \\ \hline
			\multirow{2}{*}{2} & Pole Order & 1 & 0 & 2 & 1 & 1 & 0 & 0 \\ 
			& $L^2$ & $\xmark$ &  & $\cmark$ & $\xmark$ & $\cmark$ &  &   \\ \hline
			\multirow{2}{*}{3} & Pole Order & 0 & 1 & 1 & 0 & 0 & 0 & 0 \\ 
			& $L^2$ &  & $\xmark$ & $\cmark$ &  &  &  &   \\ \hline
			\multirow{2}{*}{4} & Pole Order & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
			& $L^2$ & $\cmark$ &  &  &  &  &  &   \\ \hline
		\end{tabular}
	\end{table}
	
	
	
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_5$& $1$ & $\frac{3}{2}$ & $2$ & $3$ & $4$ & $5$ \\ \hline
			\multirow{2}{*}{1} & Pole Order & 3 & 1 & 2 & 2 & 1 & 1 \\ 
			& $L^2$ & $\cmark$ & $\xmark$ & $\xmark$ & $\cmark$ & $\xmark$ & $\cmark$  \\ \hline
			\multirow{2}{*}{2} & Pole Order & 1 & 1 & 1 & 0 & 0 & 0 \\ 
			& $L^2$ & $\xmark$ & $\xmark$ & $\cmark$ &  &  &   \\ \hline
			\multirow{2}{*}{3} & Pole Order & 1 & 0 & 0 & 0 & 0 & 0 \\ 
			& $L^2$ & $\cmark$ &  &  &  &  &   \\ \hline
		\end{tabular}
	\end{table}
	
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_6$ & $\frac{1}{2}$ & $\frac{5}{2}$ & $\frac{7}{2}$ & $\frac{11}{2}$ & $\frac{13}{2}$ \\ \hline
			\multirow{2}{*}{1} & Pole Order & 1 & 2 & 1 & 1 & 1 \\ 
			& $L^2$ & $\cmark$ & $\cmark$ & $\cmark$ & $\xmark$ & $\cmark$ \\ \hline
			\multirow{2}{*}{2} & Pole Order & 1 & 1 & 0 & 0 & 0 \\ 
			& $L^2$ & $\cmark$ & $\cmark$ & & & \\ \hline
		\end{tabular}
	\end{table}
	
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_7$ & $1$ & $5$ & $9$ \\ \hline
			\multirow{2}{*}{1} & Pole Order & 1 & 1 & 1 \\ 
			& $L^2$ & $\cmark$ & $\cmark$ & $\cmark$ \\ \hline
		\end{tabular}
	\end{table}
	
\end{Thm}

\begin{Rem}
	In the case of $E_7$ and $P=P_7$, our results agree with the results of \cite{hanzer_savin_2019}.
\end{Rem}


\begin{proof}
	The proof in this case is similar to that of $E_6$ with a few exceptional cases.
	We start with the cases that can be completely sorted using the methods of \Cref{Section:Poles_Method} and then deal with the exceptional cases.
	
	In each case $\bk{P_i,s_0,ord\bk{\chi}}$, we list the maximal order of pole of any particular intertwining operator in the following table:
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_1$& $\frac{1}{2}$ & $\frac{3}{2}$ & $\frac{5}{2}$ & $\frac{7}{2}$ & $\frac{9}{2}$ & $\frac{11}{2}$ & $\frac{13}{2}$ & $\frac{15}{2}$ & $\frac{17}{2}$ \\ \hline
			1 & Pole Order & 4 & 3 & 3 & 3 & 2 & 2 & 1 & 1 & 1 \\ \hline
			2 & Pole Order & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
		\end{tabular}
	\end{table}
	
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_2$ & $\frac{1}{2}$ & $1$ & $\frac{3}{2}$ & $2$ & $3$ & $4$ & $5$ & $6$ & $7$ \\ \hline
			1 & Pole Order & 1 & 6 & 1 & 5 & 4 & 3 & 2 & 1 & 1 \\ \hline
			2 & Pole Order & 1 & 1 & 1 & 1 & 0 & 0 & 0 & 0 & 0 \\ \hline
		\end{tabular}
	\end{table}
	
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_3$ & $\frac{1}{6}$ & $\frac{1}{2}$ & $1$ & $\frac{3}{2}$ & $2$ & $\frac{5}{2}$ & $\frac{7}{2}$ & $\frac{9}{2}$ & $\frac{11}{2}$ \\ \hline
			1 & Pole Order & 1 & 9 & 2 & 7 & 1 & 5 & 3 & 2 & 1 \\ \hline
			2 & Pole Order & 0 & 3 & 2 & 2 & 1 & 1 & 0 & 0 & 0 \\ \hline
			3 & Pole Order & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
		\end{tabular}
	\end{table}
	
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_4$ & $\frac{1}{4}$ & $\frac{1}{3}$ & $\frac{1}{2}$ & $\frac{2}{3}$ & $1$ & $\frac{3}{2}$ & $2$ & $3$ & $4$ \\ \hline
			1 & Pole Order & 1 & 2 & 5 & 2 & 11 & 2 & 6 & 3 & 1 \\ \hline
			2 & Pole Order & 1 & 0 & 5 & 0 & 4 & 2 & 1 & 0 & 0 \\ \hline
			3 & Pole Order & 0 & 2 & 0 & 2 & 1 & 0 & 0 & 0 & 0 \\ \hline
			4 & Pole Order & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
		\end{tabular}
	\end{table}
	
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_5$ & $\frac{1}{3}$ & $\frac{1}{2}$ & $\frac{2}{3}$ & $1$ & $\frac{3}{2}$ & $2$ & $3$ & $4$ & $5$ \\ \hline
			1 & Pole Order & 1 & 3 & 1 & 10 & 2 & 6 & 4 & 2 & 1 \\ \hline
			2 & Pole Order & 0 & 3 & 0 & 3 & 2 & 1 & 0 & 0 & 0 \\ \hline
			3 & Pole Order & 1 & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 0 \\ \hline
		\end{tabular}
	\end{table}
	
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_6$ & $\frac{1}{2}$ & $1$ & $\frac{3}{2}$ & $2$ & $\frac{5}{2}$ & $\frac{7}{2}$ & $\frac{9}{2}$ & $\frac{11}{2}$ & $\frac{13}{2}$ \\ \hline
			1 & Pole Order & 6 & 1 & 5 & 1 & 5 & 3 & 2 & 2 & 1 \\ \hline
			2 & Pole Order & 2 & 1 & 1 & 1 & 1 & 0 & 0 & 0 & 0 \\ \hline
		\end{tabular}
	\end{table}
	
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_7$ &$1$ & $2$ & $3$ & $4$ & $5$ & $6$ & $7$ & $8$ & $9$ \\ \hline
			1 & Pole Order & 3 & 2 & 2 & 2 & 2 & 1 & 1 & 1 & 1 \\ \hline
		\end{tabular}
	\end{table}
	
	For all cases with trivial $\chi$, the proof continues as in the case of $E_6$, with the exception of the case $\DPS{P_2}\bk{1}$, which is not generated by its spherical vector.
	This case will be dealt with bellow.
	
	We now deal with the cases with non-trivial $\chi$:
	\begin{itemize}
		\item In the following cases, there exists a singleton equivalence class which realize a pole of the same order as prescribed in the theorem and the above tables:
		$\bk{1,1/2,2}$, $\bk{3,1/2,3}$, $\bk{3,5/2,2}$, $\bk{4, 1, 3}$, $\bk{4, 2, 2}$ and $\bk{5, 1, 3}$.
		
		\item In the following cases, the pole in these tables cancels completely and the Eisenstein series is holomorphic at the point:
		$\bk{2,1/2,2}$, $\bk{2,1,2}$, $\bk{2,3/2,2}$, $\bk{3,1,2}$, $\bk{3,2,2}$, $\bk{3,1/6,3}$, $\bk{4,1/4,2}$, $\bk{4,1/3,3}$, $\bk{4,1/4,4}$, $\bk{5,1/3,3}$, $\bk{5,2/3,3}$, $\bk{6,1,2}$, $\bk{6,3/2,2}$ and $\bk{6,2,2}$.
		
		
		
		These are precisely the cases $[i,s,ord\bk{\chi}]$ in the above tables where $\DPS{P_i}\bk{s,\chi}_v$ is irreducible at infinitely many $v\in\Places$.
		
		\item In the following cases, the pole reduces to a simple pole and a simple pole is realized by a singleton equivalence class:
		$\bk{3,1/2,2}$, $\bk{3, 3/2, 2}$, $\bk{4,1,2}$, $\bk{4, 3/2, 2}$, $\bk{4, 2/3, 3}$, $\bk{5,1,2}$, $\bk{5, 3/2, 2}$, $\bk{6, 1/2, 2}$ and $\bk{6, 5/2, 2}$.
		
		\item The cases $\bk{2,2,2}$, $\bk{5,2,2}$ and $\bk{4,1/2,4}$ are dealt with in  \Cref{Chap:Square_Integrable}.
	\end{itemize}
	
	
	
	
	These leaves the case of $\bk{2,1,1}$ to be treated.
	
	
	
	In the case of $\bk{2,1,1}$ the method outlined in \Cref{Section:Poles_Method} requires a few modifications.
	We recall that $\DPS{P_2}\bk{1}$ has the following structure
	\[
	\pi_{s,v} \hookrightarrow \DPS{P_2}\bk{1}_v \twoheadrightarrow \pi_{1,v}\oplus\pi_{-1,v},
	\]
	where $\pi_0$ is the unique irreducible spherical subquotient and $\pi_{-1}$ is irreducible but not spherical.
	Furthermore,
	\[
	\dim_\C\pi_{-1,v}^{\frakJ_v} = 15 .
	\]
	Let
	\[
	\lambda_{0,v} = \esevenchar{-1}{5}{-1}{-1}{-1}{-1}{-1}
	\]
	denote the initial exponent of $\DPS{P_2}\bk{-1}$.
	Then, we may write
	\[
	r_{T_v}^{G_v}\pi_{-1,v} = \oplus_{\lambda\in Y} w\cdot\lambda_{0,v},
	\]
	where $Y\subset W$ is independent of $v$ and satisfies $\Card{Y}=15$.
	In particular, we note that $\Card{\coset{w}}=2$ for $w\in Y$.
	Furthermore,
	\[
	M_w\bk{\lambda_{s}^{P_2}} f_s\bk{g}
	= C_w\bk{\lambda_{s}^{P_2}} \otimes_{v\notin S}f_{s,v}\bk{g_v} \otimes_{v\in S} N_{w,v}\bk{\lambda_{s}^{P_2}}f_{s,v}\bk{g_v} 
	\]
	and
	\[
	N_{w,v}\bk{\lambda_{-1}^{P_2}}f_{s,v}\bk{g_v} \in i_{T_v}^{G_v}w\cdot\lambda_0 = i_{T_v}^{G_v}w\cdot\lambda_{-1}^{P_2} .
	\]
	Hence, $\pi_{1,v}$ appears in the image of $N_{w,v}\bk{\lambda_{s}^{P}}$ only for $w\in W^{M,T}$ such that $w\in Y$.
	In particular, one checks that for any other $w\in W^{M,T}$ such that $\kappa_{\coset{w}}$ admits a pole at $s_0=1$, it holds that $\Image\bk{N_{w,v}\bk{\lambda_{1}^{P}}}=\pi_{1,v}$.
	
	Hence, the order of $\kappa_{\coset{w}}$ at $s_0=1$ for $w\in W^{M,T} \setminus Y$ such that $\kappa_{\coset{w}}$ admits a pole there, is bounded by the order of $\kappa_{\coset{w}}\bk{f^0,g}$ there.
	Since
	\[
	\kappa_{\coset{w}}\bk{f^0,g,s} = \suml_{w\in W^{M,T}} C_w\bk{\lambda_{s,\chi}^{P_2}},
	\]
	the order of $\kappa_{\coset{w}}\bk{f^0,g}$ at $s_0=1$ can be determined by a standard calculation.
	Furthermore, one may use the method described in \Cref{Subsection:Poles_Method_Normalized_Eis_ser}, in order to show that $\kappa_{\coset{w}}\bk{f^0,g}$ admits at most a simple pole at $s_0=1$.
	
	
	
\end{proof}




\section{Results for $E_8$}


\begin{table}
	\centering
	\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|}
		\hline
		$ord\bk{\chi}$ & $P_1$& $\frac{1}{2}$ & $\frac{5}{2}$ & $\frac{7}{2}$ & $\frac{11}{2}$ & $\frac{13}{2}$ & $\frac{17}{2}$ & $\frac{23}{2}$ \\ \hline
		\multirow{2}{*}{1} & Pole Order & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ 
		& $L^2$ & $\cmark$ & $\cmark$ & $\cmark$ & $\xmark$ & $\cmark$ & $\cmark$ & $\cmark$  \\ \hline
		\multirow{2}{*}{2} & Pole Order & 1 & 0 & 1 & 0 & 0 & 0 & 0 \\ 
		& $L^2$ & \cmark &  & \cmark &  &  &  &   \\ \hline
	\end{tabular}
\end{table}


\begin{table}
	\centering
	\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|c|}
		\hline
		$ord\bk{\chi}$ & $P_2$& $\frac{1}{2}$ & $\frac{3}{2}$ & $\frac{5}{2}$ & $\frac{7}{2}$ & $\frac{9}{2}$ & $\frac{11}{2}$ & $\frac{13}{2}$ & $\frac{17}{2}$ \\ \hline
		\multirow{2}{*}{1} & Pole Order & 1 & 2 & 2 & 2 & 1 & 1 & 1 & 1 \\ 
		& $L^2$ & $\cmark$ & $\cmark$ & $\cmark$ & $\cmark$ & $\xmark$ & $\xmark$ & $\cmark$ & $\cmark$  \\ \hline
		\multirow{2}{*}{2} & Pole Order & 1 & 1 & 1 & 1 & 0 & 0 & 0 & 0 \\ 
		& $L^2$ & \cmark & \cmark & \cmark & \cmark &  &  &  &  \\ \hline
		\multirow{2}{*}{3} & Pole Order & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
		& $L^2$ &  & \cmark &  &  &  &  &  &  \\ \hline
	\end{tabular}
\end{table}

\begin{table}
	\centering
	\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|c|c|c|}
		\hline
		$ord\bk{\chi}$ & $P_3$& $\frac{1}{2}$ & $1$ & $\frac{7}{6}$ & $\frac{3}{2}$ & $2$ & $\frac{5}{2}$ & $\frac{7}{2}$ & $\frac{9}{2}$ & $\frac{11}{2}$ & $\frac{13}{2}$ \\ \hline
		\multirow{2}{*}{1} & Pole Order & 1 & 1 & 1 & 3 & 1 & 2 & 2 & 1 & 1 & 1 \\ 
		& $L^2$ & $\xmark$ & $\xmark$ & $\xmark$ & $\cmark$ & $\xmark$ & $\cmark$ & $\cmark$ & $\xmark$ & $\xmark$ & $\cmark$  \\ \hline
		\multirow{2}{*}{2} & Pole Order & 1 & 1 & 0 & 1 & 1 & 1 & 1 & 0 & 0 & 0 \\ 
		& $L^2$ & \cmark & \xmark &  & \xmark & \xmark & \cmark & \cmark &  &  &  \\ \hline
		\multirow{2}{*}{3} & Pole Order & 0 & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
		& $L^2$ &  &  & \xmark & \cmark &  &  &  &  &  &  \\ \hline
		\multirow{2}{*}{4} & Pole Order & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
		& $L^2$ &  & \cmark &  &  &  &  &  &  &  &  \\ \hline
	\end{tabular}
\end{table}


\begin{table}
	\centering
	\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
		\hline
		$ord\bk{\chi}$ & $P_4$& $\frac{3}{10}$ & $\frac{1}{2}$ & $\frac{3}{4}$ & $\frac{5}{6}$ & $1$ & $\frac{7}{6}$ & $\frac{3}{2}$ & $2$ & $\frac{5}{2}$ & $\frac{7}{2}$ & $\frac{9}{2}$ \\ \hline
		\multirow{2}{*}{1} & Pole Order & 1 & 5 & 1 & 1 & 2 & 1 & 4 & 1 & 3 & 2 & 1 \\ 
		& $L^2$ & $\xmark$ & $\cmark$ & $\xmark$ & $\xmark$ & $\xmark$ & $\xmark$ & $\cmark$ & $\xmark$ & $\cmark$ & $\cmark$ & $\cmark$  \\ \hline
		\multirow{2}{*}{2} & Pole Order & 0 & 3 & 1 & 0 & 2 & 0 & 2 & 1 & 1 & 0 & 0  \\
		& $L^2$ &  & \cmark & \xmark &  & \xmark &  & \cmark & \xmark & \cmark &  &  \\ \hline
		\multirow{2}{*}{3} & Pole Order & 0 & 2 & 0 & 1 & 0 & 1 & 1 & 0 & 0 & 0 & 0  \\
		& $L^2$ &  & \cmark &  & \xmark &  & \xmark & \cmark &  &  &  &  \\ \hline
		\multirow{2}{*}{4} & Pole Order & 0 & 1 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0  \\
		& $L^2$ &  & \xmark & \xmark &  & \cmark &  &  &  &  &  &  \\ \hline
		\multirow{2}{*}{5} & Pole Order & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0  \\
		& $L^2$ & \xmark & \cmark &  &  &  &  &  &  &  &  &  \\ \hline
		\multirow{2}{*}{6} & Pole Order & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0  \\
		& $L^2$ &  & \cmark &  &  &  &  &  &  &  &  &  \\ \hline
	\end{tabular}
\end{table}


\begin{table}
	\centering
	\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|c|c|c|}
		\hline
		$ord\bk{\chi}$ & $P_5$& $\frac{1}{2}$ & $\frac{5}{6}$ & $1$ & $\frac{7}{6}$ &  $\frac{3}{2}$ & $2$ & $\frac{5}{2}$ & $\frac{7}{2}$ & $\frac{9}{2}$ & $\frac{11}{2}$ \\ \hline
		\multirow{2}{*}{1} & Pole Order & 4 & 1 & 2 & 1 & 4 & 1 & 3 & 2 & 1 & 1 \\ 
		& $L^2$ & $\cmark$ & $\xmark$ & $\xmark$ & $\xmark$ & $\cmark$ & $\xmark$ & $\cmark$ & $\cmark$ & $\xmark$ & $\cmark$  \\ \hline
		\multirow{2}{*}{2} & Pole Order & 2 & 0 & 2 & 0 & 2 & 1 & 1 & 0 & 0 & 0 \\ 
		& $L^2$ & \cmark &  & \cmark &  & \cmark & \xmark & \cmark &  &  &   \\ \hline
		\multirow{2}{*}{3} & Pole Order & 1 & 1 & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 0 \\ 
		& $L^2$ & \xmark & \xmark &  & \xmark & \cmark &  &  &  &  &   \\ \hline
		\multirow{2}{*}{4} & Pole Order & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
		& $L^2$ & \cmark &  & \cmark &  &  &  &  &  &  &   \\ \hline
		\multirow{2}{*}{5} & Pole Order & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
		& $L^2$ & \cmark &  &  &  &  &  &  &  &  &   \\ \hline
	\end{tabular}
\end{table}



\begin{table}
	\centering
	\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|c|c|c|}
		\hline
		$ord\bk{\chi}$ & $P_6$& $\frac{1}{2}$ & $1$ & $2$ & $\frac{5}{2}$ & $3$ & $4$ & $5$ & $6$ & $7$ \\ \hline
		\multirow{2}{*}{1} & Pole Order & 1 & 2 & 3 & 1 & 2 & 1 & 1 & 1 & 1 \\ 
		& $L^2$ & $\xmark$ & $\cmark$ & $\cmark$ & $\xmark$ & $\cmark$ & $\xmark$ & $\xmark$ & $\xmark$ & $\cmark$  \\ \hline
		\multirow{2}{*}{2} & Pole Order & 1 & 1 & 1 & 1 & 1 & 0 & 0 & 0 & 0 \\ 
		& $L^2$ & \cmark & \cmark & \xmark & \xmark & \cmark &  &  &  &   \\ \hline
		\multirow{2}{*}{3} & Pole Order & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
		& $L^2$ &  & \cmark & \cmark &  &  &  &  &  &   \\ \hline
		\multirow{2}{*}{4} & Pole Order & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
		& $L^2$ & \cmark &  &  &  &  &  &  &  &   \\ \hline
	\end{tabular}
\end{table}


\begin{table}
	\centering
	\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|}
		\hline
		$ord\bk{\chi}$ & $P_7$& $\frac{1}{2}$ & $\frac{3}{2}$ & $\frac{5}{2}$ & $\frac{9}{2}$ & $\frac{11}{2}$ & $\frac{17}{2}$ & $\frac{19}{2}$ \\ \hline
		\multirow{2}{*}{1} & Pole Order & 2 & 1 & 1 & 2 & 1 & 1 & 1 \\ 
		& $L^2$ & $\cmark$ & $\cmark$ & $\cmark$ & $\cmark$ & $\cmark$ & $\xmark$ & $\cmark$  \\ \hline
		\multirow{2}{*}{2} & Pole Order & 1 & 0 & 1 & 1 & 0 & 0 & 0 \\ 
		& $L^2$ & \cmark &  & \cmark & \cmark &  &  &   \\ \hline
		\multirow{2}{*}{3} & Pole Order & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
		& $L^2$ & \cmark &  &  &  &  &  &   \\ \hline
	\end{tabular}
\end{table}

\begin{table}
	\centering
	\begin{tabular}[H]{|c|c|c|c|c|c|}
		\hline
		$ord\bk{\chi}$ & $P_8$& $\frac{1}{2}$ & $\frac{11}{2}$ & $\frac{19}{2}$ & $\frac{29}{2}$ \\ \hline
		\multirow{2}{*}{1} & Pole Order & 1 & 1 & 1 & 1 \\ 
		& $L^2$ & $\cmark$ & $\cmark$ & $\cmark$ & $\cmark$ \\ \hline
		\multirow{2}{*}{2} & Pole Order & 1 & 0 & 0 & 0 \\ 
		& $L^2$ & \cmark &  &  &  \\ \hline
	\end{tabular}
\end{table}



\begin{proof}
	As in the previous cases, we start by recording the maximal order of pole of any particular intertwining operator, for each case $\bk{P_i,s_0,ord\bk{\chi}}$, in the following table:
	%	\newpage
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_1$& $\frac{1}{2}$ & $1$ & $\frac{3}{2}$ & $2$ & $\frac{5}{2}$ & $3$ & $\frac{7}{2}$ & $\frac{9}{2}$ & $\frac{11}{2}$ & $\frac{13}{2}$ & $\frac{15}{2}$ & $\frac{17}{2}$ & $\frac{19}{2}$ & $\frac{21}{2}$ & $\frac{23}{2}$ \\ \hline
			1 & Pole Order & 7 & 1 & 6 & 1 & 6 & 1 & 5 & 4 & 4 & 3 & 2 & 2 & 1 & 1 & 1 \\ \hline
			2 & Pole Order & 2 & 1 & 1 & 1 & 1 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
		\end{tabular}
	\end{table}
	
	
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_2$ & $\frac{1}{6}$ & $\frac{1}{2}$ & $\frac{5}{6}$ & $1$ & $\frac{7}{6}$ & $\frac{3}{2}$ & $2$ & $\frac{5}{2}$ & $3$ & $\frac{7}{2}$ & $\frac{9}{2}$ & $\frac{11}{2}$ & $\frac{13}{2}$ & $\frac{15}{2}$ & $\frac{17}{2}$ \\ \hline
			1 & Pole Order & 1 & 11 & 1 & 3 & 1 & 10 & 2 & 8 & 1 & 6 & 4 & 3 & 2 & 1 & 1 \\ \hline
			2 & Pole Order & 0 & 4 & 0 & 3 & 0 & 3 & 2 & 2 & 1 & 1 & 0 & 0 & 0 & 0 & 0 \\ \hline
			3 & Pole Order & 1 & 1 & 1 & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
		\end{tabular}
	\end{table}	
	
	
	
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_3$ & $\frac{1}{6}$ & $\frac{1}{4}$ & $\frac{1}{2}$ & $\frac{3}{4}$ & $\frac{5}{6}$ & $1$ & $\frac{7}{6}$ & $\frac{3}{2}$ & $2$ & $\frac{5}{2}$ & $3$ & $\frac{7}{2}$ & $\frac{9}{2}$ & $\frac{11}{2}$ & $\frac{13}{2}$ \\ \hline
			1 & Pole Order & 2 & 1 & 14 & 1 & 2 & 5 & 2 & 11 & 3 & 7 & 1 & 5 & 3 & 2 & 1 \\ \hline
			2 & Pole Order & 0 & 1 & 6 & 1 & 0 & 5 & 0 & 4 & 3 & 2 & 1 & 1 & 0 & 0 & 0 \\ \hline
			3 & Pole Order & 2 & 0 & 2 & 0 & 2 & 0 & 2 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
			4 & Pole Order & 0 & 1 & 1 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
		\end{tabular}
	\end{table}	
	
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_4$ & $\frac{1}{10}$ & $\frac{1}{6}$ & $\frac{1}{4}$ & $\frac{3}{10}$ & $\frac{1}{3}$ & $\frac{1}{2}$ & $\frac{3}{4}$ & $\frac{5}{6}$ & $1$ & $\frac{7}{6}$ & $\frac{3}{2}$ & $2$ & $\frac{5}{2}$ & $\frac{7}{2}$ & $\frac{9}{2}$ \\ \hline
			1 & Pole Order & 2 & 5 & 3 & 2 & 1 & 21 & 2 & 3 & 6 & 2 & 11 & 2 & 6 & 3 & 1 \\ \hline
			2 & Pole Order & 0 & 1 & 3 & 0 & 1 & 10 & 2 & 0 & 6 & 0 & 4 & 2 & 1 & 0 & 0 \\ \hline
			3 & Pole Order & 0 & 5 & 0 & 0 & 1 & 5 & 0 & 3 & 0 & 2 & 1 & 0 & 0 & 0 & 0 \\ \hline
			4 & Pole Order & 0 & 0 & 3 & 0 & 0 & 3 & 2 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
			5 & Pole Order & 2 & 0 & 0 & 2 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
			6 & Pole Order & 0 & 1 & 0 & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
		\end{tabular}
	\end{table}	
	
	
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_5$ & $\frac{1}{10}$ & $\frac{1}{6}$ & $\frac{1}{4}$ & $\frac{3}{10}$ & $\frac{1}{2}$ & $\frac{3}{4}$ & $\frac{5}{6}$ & $1$ & $\frac{7}{6}$ & $\frac{3}{2}$ & $2$ & $\frac{5}{2}$ & $\frac{7}{2}$ & $\frac{9}{2}$ & $\frac{11}{2}$ \\ \hline
			1 & Pole Order & 1 & 4 & 2 & 1 & 20 & 1 & 3 & 6 & 2 & 12 & 2 & 7 & 4 & 2 & 1 \\ \hline
			2 & Pole Order & 0 & 0 & 2 & 0 & 8 & 1 & 0 & 6 & 0 & 4 & 2 & 1 & 0 & 0 & 0 \\ \hline
			3 & Pole Order & 0 & 4 & 0 & 0 & 4 & 0 & 3 & 0 & 2 & 1 & 0 & 0 & 0 & 0 & 0 \\ \hline
			4 & Pole Order & 0 & 0 & 2 & 0 & 2 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
			5 & Pole Order & 1 & 0 & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
		\end{tabular}
	\end{table}
	
	
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_6$ & $\frac{1}{4}$ & $\frac{1}{3}$ & $\frac{1}{2}$ & $\frac{2}{3}$ & $1$ & $\frac{4}{3}$ & $\frac{3}{2}$ & $\frac{5}{3}$ & $2$ & $\frac{5}{2}$ & $3$ & $4$ & $5$ & $6$ & $7$ \\ \hline
			1 & Pole Order & 1 & 2 & 5 & 2 & 12 & 1 & 3 & 1 & 10 & 2 & 6 & 4 & 3 & 2 & 1 \\ \hline
			2 & Pole Order & 1 & 0 & 5 & 0 & 4 & 0 & 3 & 0 & 3 & 2 & 1 & 0 & 0 & 0 & 0 \\ \hline
			3 & Pole Order & 0 & 2 & 0 & 2 & 2 & 1 & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
			4 & Pole Order & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
		\end{tabular}
	\end{table}	
	
	
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_7$ & $\frac{1}{6}$ & $\frac{1}{2}$ & $1$ &$\frac{3}{2}$ & $2$ & $\frac{5}{2}$ & $3$ & $\frac{7}{2}$ & $4$ & $\frac{9}{2}$ & $\frac{11}{2}$ & $\frac{13}{2}$ & $\frac{15}{2}$ & $\frac{17}{2}$ & $\frac{19}{2}$ \\ \hline
			1 & Pole Order & 1 & 9 & 2 & 7 & 2 & 6 & 1 & 5 & 1 & 5 & 3 & 2 & 2 & 2 & 1 \\ \hline
			2 & Pole Order & 0 & 3 & 2 & 2 & 2 & 2 & 1 & 1 & 1 & 1 & 0 & 0 & 0 & 0 & 0 \\ \hline
			3 & Pole Order & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
		\end{tabular}
	\end{table}	
	
	
	
	\begin{table}
		\centering
		\begin{tabular}[H]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
			$ord\bk{\chi}$ & $P_8$& $\frac{1}{2}$ & $\frac{3}{2}$ & $\frac{5}{2}$ & $\frac{7}{2}$ & $\frac{9}{2}$ & $\frac{11}{2}$ & $\frac{13}{2}$ & $\frac{15}{2}$ & $\frac{17}{2}$ & $\frac{19}{2}$ & $\frac{21}{2}$ & $\frac{23}{2}$ & $\frac{25}{2}$ & $\frac{27}{2}$ & $\frac{29}{2}$ \\ \hline
			1 & Pole Order & 4 & 3 & 3 & 3 & 3 & 3 & 2 & 2 & 2 & 2 & 1 & 1 & 1 & 1 & 1 \\ \hline
			2 & Pole Order & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
		\end{tabular}
	\end{table}
	
	
	
	For all cases with trivial $\chi$, the proof continues as in the case of $E_6$, with the exception of the cases:
	\begin{itemize}
		\item  $\DPS{P_1}\bk{\frac{5}{2}}$ and $\DPS{P_7}\bk{\frac{3}{2}}$ which are not generated by its spherical vector.
		\item $\DPS{P_2}\bk{\frac{1}{2}}$ and $\DPS{P_5}\bk{\frac{1}{2}}$ for whom the length of the local maximal semi-simple quotient is not yet determined.
	\end{itemize}
	These cases will be dealt with bellow.
	
	We now deal with the cases with non-trivial $\chi$:
	\begin{itemize}
		\item In the following cases, there exists a singleton equivalence class which realize a pole of the same order as prescribed in the theorem and the above tables:
		$\bk{1,7/2,2}$, $\bk{2,7/2,2}$, $\bk{2,3/2,3}$, $\bk{3,7/2,2}$, $\bk{3,3/2,3}$, $\bk{3,1,4}$, $\bk{4,5/2,2}$, $\bk{4,3/2,3}$, $\bk{4,1,4}$, $\bk{4,1/2,5}$, $\bk{4,1/2,6}$, $\bk{5,5/2,2}$, $\bk{5,3/2,3}$, $\bk{5,1,4}$, $\bk{5,1/2,5}$, $\bk{6,3,2}$, $\bk{6,2,3}$, $\bk{6,1/2,4}$, $\bk{7,9/2,2}$, $\bk{7,1/2,3}$ and $\bk{8,1/2,2}$.
		.
		
		\item In the following cases, the pole in these tables cancels completely and the Eisenstein series is holomorphic at the point, sorted by the value of $i$:
		\begin{enumerate}
			\item $\bk{1,1,2}$, $\bk{1,3/2,2}$, $\bk{1,2,2}$, $\bk{1,5/2,2}$ and $\bk{1,3,2}$.
			\item $\bk{2,3,2}$, $\bk{2,2,2}$, $\bk{2,1/6,3}$, $\bk{2,1/2,3}$, $\bk{2,5/6,3}$ and $\bk{2,7/6,3}$.
			\item $\bk{3,3,2}$, $\bk{3,3/4,2}$, $\bk{3,1/4,2}$, $\bk{3,3,2}$, $\bk{3,1/6,3}$, $\bk{3,1/2,3}$ and $\bk{3,5/6,3}$.
			\item $\bk{4,1/3,2}$, $\bk{4,1/6,2}$, $\bk{4,1/3,3}$, $\bk{4,1/10,5}$, $\bk{4,1/6,6}$ and $\bk{4,1/3,6}$.
			\item $\bk{5,1/4,2}$, $\bk{5,3/4,2}$, $\bk{5,1/4,4}$, $\bk{5,3/4,4}$, $\bk{5,1/10,5}$ and $\bk{5,3/10,5}$.
			\item $\bk{6,1/4,2}$, $\bk{6,4/3,3}$, $\bk{6,1/3,3}$, $\bk{6,2/3,3}$, $\bk{6,5/3,3}$ and $\bk{6,1/4,4}$.
			\item $\bk{7,1,2}$, $\bk{7,3/2,2}$, $\bk{7,2,2}$, $\bk{7,3,2}$, $\bk{7,7/2,2}$, $\bk{7,4,2}$ and $\bk{7,1/6,3}$.
		\end{enumerate}
		
		\redcolor{Still missing the cases: [2,1,2], [4,1/4,2], [4,1/6,3], [4,1/4,4], [5,1/6,3], [6,3/2,2] .	
			\todonum{Remaining cases: order of poles, $E_8$ case, from old code}
			
		}
		
		These are precisely the cases $[i,s,ord\bk{\chi}]$ in the above tables where $\DPS{P_i}\bk{s,\chi}_v$ is irreducible at infinitely many $v\in\Places$.
		
		\item In the following cases, the pole reduces to a simple pole and a simple pole is realized by a singleton equivalence class, sorted by the value of $i$:
		\begin{enumerate}
			\item $\bk{1,1/2,2}$.
			\item $\bk{2,3/2,2}$, $\bk{2,5/2,2}$ and $\bk{2,7/2,2}$.
			\item $\bk{3,2,2}$, $\bk{3,5/2,2}$ and $\bk{3,7/6,3}$.
			\item $\bk{4,1/2,4}$, $\bk{4,3/4,2}$, $\bk{4,3/2,2}$, $\bk{4,1,2}$, $\bk{4,2,2}$, $\bk{4,1/2,3}$, $\bk{4,5/6,3}$, $\bk{4,7/6,3}$, $\bk{4,3/4,4}$ and $\bk{4,3/10,5}$.
			\item $\bk{5,1,2}$, $\bk{5,3/2,2}$, $\bk{5,2,2}$, $\bk{5,5/6,3}$, $\bk{5,7/6,3}$ and $\bk{5,1/2,4}$.
			\item $\bk{6,1/2,2}$, $\bk{6,2,2}$, $\bk{6,5/2,2}$ and $\bk{6,1,3}$.
			\item $\bk{7,1/2,2}$ and $\bk{7,5/2,2}$
		\end{enumerate}
		
		\redcolor{Still missing the cases: [2,1/2,2], [3,1,2], [3,3/2,2], [4,1/2,2], [5,1/2,2], [5,1/2,3], [6,1,2].
			
			Special case (Co-socle of length $2$): [3,1/2,2].
			
			Solved using $A_6$,$D_6$ special cases: [4,1,2], [4,1/2,3], [5,1,2], [6,1/2,2].
		}
		
		
	\end{itemize}
	
\end{proof}


It should be noted that the results of this section settles a conjecture made by David Ginzburg and Joseph Hundley in \cite{MR3359720}.

\begin{Conj}[\cite{MR3359720}, Conjecture 2]
	For $\Real\bk{s}>0$, the possible poles of the Eisenstein series $\Eisen_{P_2}^{E_8}\bk{s,\chi}$ are as follows.
	\begin{itemize}
		\item If $\chi$ is trivial, then the Eisenstein series $\Eisen_{P_2}\bk{s,\chi}$ can have a double pole at the points $\frac{3}{2}$, $\frac{5}{2}$ and $\frac{7}{2}$.
		At the points $\frac{1}{2}$, $\frac{9}{2}$, $\frac{11}{2}$, $\frac{13}{2}$ and $\frac{17}{2}$ it can have a simple pole.
		\item If $\chi$ is nontrivial quadratic, then the Eisenstein series can have simple poles at
		$\frac{1}{2}$, $\frac{3}{2}$, $\frac{5}{2}$ and $\frac{7}{2}$.
		\item If $\chi$ is nontrivial cubic, then the Eisenstein series can have a simple pole at $\frac{3}{2}$.
		\item If the order of $\chi$ exceeds 3 then the Eisenstein series is holomorphic in $\Real\bk{s}>0$.
	\end{itemize}
\end{Conj}

\begin{Rem}
	Note that the normalization of the variable $s$ is slightly different in \cite{MR3359720}.
	If $t_0$ is a pole in the notations of \cite{MR3359720}, then the corresponding value $s_0$ in our notations is
	\[
	s_0= 17\times\bk{t_0-\frac{1}{2}} .
	\]
\end{Rem}

==> sec-Arthur_-_Copy.tex <==
\chapter[Arthur Parameters]{Arthur Parameters of the Square-Integrable Degenerate Residual Representations}
\label{Chap:Arthur}

In this chapter, we wish to compare the results of \Cref{Chap:Square_Integrable} with the Arthur conjectures  for $L^2_{\coset{\bT}}$.
We start by a brief description of Arthur parameters and conjectures.
Please see \cite{MR1021499} for more details.
Also, the reader may wish to consider \cite{MR1847140,MR1426903,MR2262172} for other detailed examples.

\section{Arthur Parameters and the Arthur Conjectures}

Arthur's conjectures aims at a precise description of the discrete spectrum $L^2_{dis.}\bk{ G\bk{F}\lmod G\bk{\AA}}$ of $G\bk{\AA}$.
More precisely, the conjectures first imply a rough decomposition
\[
L^2_{dis.}\bk{ G\bk{F}\lmod G\bk{\AA}} = \widehat{\oplus}_\psi L^2\bk{ G\bk{F} \lmod G\bk{\AA}}_\psi,
\]
where $\psi$ runs through the set of global A-parameters, that is the set of $\check{G}$-conjugacy classes of admissible maps
\[
\psi : \Lfun_F \times SL_2\bk{\C} \to \check{G} ,
\]
where $\Lfun_F$ is the conjectural Langlands group of the number field $F$.

The conjectures, then give a description of the space $L^2_\psi = L^2\bk{ G\bk{F}\lmod G\bk{\AA}}_\psi$.

First, we describe the local constituents $\pi_v$ of the irreducible constituents $\pi=\otimes_{v\in \Places}\pi_v$ of $L^2_\psi$.
Since the local Weil group $W_{F_v}$ embeds into $\Lfun_F$ (according to the conjectured properties of $\Lfun_F$), the global A-parameter $\psi$ gives rise to the local A-parameter
\todonum{Should it be Weil-Deligne group here?}
\[
\psi_v = \psi\res{W_{F_v}\times SL_2\bk{\C}} .
\]
Denote $C_{\psi_v} = Cent\bk{im \psi, \check{G}}$ and let $S_{\psi_v} = C_{\psi_v}\rmod C_{\psi_v}^0$.
$S_{\psi_v}$ is called the component group associated to $\psi$.
Note that $S_{\psi_v}$ is a finite group.

Arthur's conjectures state, among other things, that:
\begin{itemize}
	\item There exists a set of irreducible representations $\Pi_{\psi_v}$, called the local A-packet of $\psi_v$, with a bijection
	\begin{equation}
		\label{Eq:Local_Arthur_cor}
		\begin{split}
			\widehat{S_{\psi_v}} & \to  \Pi_{\psi_v} \\
			\eta_v & \mapsto  \pi_{\eta_v}
		\end{split}
	\end{equation}
	
	\item If $\eta_v = \Id_v$, then $\pi_{\eta_v}$ is unramified with Satake parameter
	\begin{equation}
		\label{Eq:Satake_parameter_for_Arthur_parameter}
		\sigma_{\psi_v} = \psi_v \bk{Fr_v, \begin{pmatrix} q_v^{\frac12} & \\ & q_v^{-\frac12} \end{pmatrix}},
	\end{equation}
	where $Fr_v$ is the Frobenius element of $W_{F_v} \hookrightarrow \Lfun_{F_v}$.
	
	\item The global A-packet of $\psi$, defined by
	\[
	\Pi_\psi = \set{\pi=\otimes_{v\in\Places} \pi_{\eta_v} \mvert \pi_{\eta_v}\in \Pi_{\psi_v}, \ \eta_v=\Id_v \text{ for almost all $v$} },
	\]
	is in bijection with with the set of irreducible representations of the compact set $S_{\psi,\AA} = \prodl_{v\in\Places} S_{\psi_v}$.
	We write this bijection as follows
	\[
	\begin{split}
		\widehat{S_{\psi,\AA}} & \to \Pi_\psi \\
		\eta = \otimes_{v\in \Places} \eta_v & \mapsto \pi_\eta =  \otimes_{v\in\Places} \pi_{\eta_v} .
	\end{split}
	\]
	Note that $S_{\psi}$ embeds diagonally into $S_{\psi,\AA}$.
	
	\item Arthur attached a quadratic character $\epsilon_\psi$ of $S_\psi$ such that, for $\eta\in \widehat{S_{\psi,\AA}}$, the multiplicity of $\eta$ in $L^2\bk{S_{\psi,\AA}}$ and of $\pi_\eta$ in $L^2_{dis.}$ is given by
	\begin{equation}
		\label{Eq:Arthurs_multiplicity_formula}
		m_\eta = \frac{1}{\Card{S_\psi}} \bk{\suml_{s\in S_\psi} \epsilon_\psi \bk{s} \cdot \eta\bk{s}} .
	\end{equation}
	In particular, if $\mu=1$, then $\epsilon_\psi=1$.
	\item In particular, if $S_{\psi}$ is finite (in which case, $\psi$ is called \emph{elliptic}), then $\pi_\eta=\otimes \pi_{\eta_v}$ occurs in the discrete spectrum if and only if
	\begin{equation}
		\label{Eq:Arthur_test_for_discrete_series}
		\suml_{s\in S_\psi} \prodl_{v\in\Places}\eta_v\bk{s_v}  \neq 0 ,
	\end{equation}
	where we write $s=\otimes s_v$.
\end{itemize}

In order to analyze an Arthur parameter $\psi: \Lfun_F \times SL_2\bk{\C} \to \check{G}$, we need to describe the two commuting maps
\[
\begin{split}
	& \phi:SL_2\bk{\C}\to\check{G}, \quad \phi\bk{g}=\psi\bk{1,g} \\
	& \mu:\Lfun_F \to \check{G} , \quad \mu\bk{x} = \psi\bk{x,1} .
\end{split}
\]
First of all, we note that, by the Jacobson-Morozov Theorem (see \cite{MR1503258,MR0007750}), the $\check{G}$-conjugacy class of $\phi$ is determined by $X = \phi\begin{pmatrix} 1&1\\0&1 \end{pmatrix}$.
%\begin{Thm}[Jacobson-Morozov Theorem \cite{MR1503258,MR0007750}]
%	Suppose that $u$ is a unipotent element in a semi-simple algebraic group $G$.
%	Then, there exists a homomorphism $\phi:SL_2\bk{\C}\to G$ such that $\phi\begin{pmatrix} 1&1\\0&1 \end{pmatrix} = u$.
%\end{Thm}

After fixing $X$ and $\phi$, we note that $\mu$ is, in fact, a map $\mu:\Lfun_F \to C_\phi$, where $C_\phi = Cent\bk{im\ \phi, \check{G}}$.

We also write $C_X = Cent\bk{X, \check{G}}$ and let $U^X$ denote the unipotent radical of $U_X$.
By \cite[Proposition 2.4]{MR782556}, it holds that
\begin{itemize}
	\item $C_\phi$ is reductive and $C_X = C_\phi \cdot U^X$ is a Levi decomposition.
	\item The inclusion $C_\phi \subseteq C_X$ induces an isomorphism on the component groups, $C_\phi\rmod C_\phi^0 Z_{\check{G}} \cong C_X\rmod C_X^0 Z_{\check{G}}$.
\end{itemize}
%\begin{Lem}[\cite{MR782556}, Proposition 2.4]
%	Let $u$ be a unipotent element and $\phi:SL_2\to G$ be a homomorphism such that $\phi\begin{pmatrix} 1&1\\0&1 \end{pmatrix} = u$.
%	Let $S_\phi=Cent\bk{im \phi,G} \subset S_u=Cent\bk{u,G}$ and $U^u$ be the unipotent radical of $S_u$.
%	Then
%	\begin{enumerate}
%		\item $S_u=S_\phi\cdot U^u$, a semi-direct product. $S_\phi$ is reductive.
%		\item The inclusion $S_\phi\subset S_u$ induces an isomorphism between $S_\phi\rmod S_\phi^0 Z_G$ and $S_u\rmod S_u^0 Z_G$.
%	\end{enumerate}
%\end{Lem}



For $X$ as above, let $\gen{X, Y, H}$ be an $SL_2$-triple as in the Jacobson-Morozov theorem such that $H=\phi\begin{pmatrix} q&\\&q^{-1} \end{pmatrix}$.
%\redcolor{
%Since, $H \in im\ \phi$, and since $C_H^0=Cent\bk{H,\check{G}}^0$ is reductive, it follows that $C_H^0\subset C_\phi$.
%
%By \cite[Theorem 3.5.3]{MR1266626}, we have
%\[
%\begin{split}
%	& Cent\bk{H,\check{G}} = C_H = \gen{T; X_\alpha, \alpha\bk{X}=1 ; \dot{w}, w\cdot X=X} \\
%	& Cent\bk{H,\check{G}}^0 = C_H^0 = \gen{T, X_\alpha, \alpha\bk{X}=1},
%\end{split}
%\]
%}

We denote by $\mu_k$ the cyclic group $\ZZ\rmod\bk{k\ZZ}$ and by $S_k$ we denote the symmetric group of order $k!$.

Also, it should be added that all data regarding nilpotent orbits and their centralizers, can be read from the tables in \cite[page 402-407]{MR1266626}.


%We now turn to deal with the cases $\chi=\Id$ and $\chi\neq\Id$ separately.
%\todonum{Add $R$-groups?}

%\begin{Thm}[\cite{MR1266626}, Theorem 3.5.3]
%	Let $s$ be semi-simple and $T$ be a maximal torus of $G$ containing $s$.
%	Then
%	\begin{enumerate}
%		\item $C_G\bk{s}^{0} = \gen{T, X_\alpha, \alpha\bk{s}=1}$.
%		\item $C_G\bk{s} = \gen{T, X_\alpha, \alpha\bk{s}=1 ; \dot{w}, s^w=s}$.
%	\end{enumerate}
%\end{Thm}
%
%\begin{Thm}[\cite{MR1266626}, Theorem 3.5.4]
%	Let $s$ be semi-simple.
%	Then $C_G\bk{s}^{0}$ is reductive. Its root system is 
%	\[
%	\Phi'= \set{\alpha\in\Phi_G \mvert \alpha\bk{s}=1}
%	\]
%	and its Weyl group is
%	\[
%	W' = \gen{w_\alpha \mvert \alpha\in\Phi'} .
%	\]
%\end{Thm}

%%For a split group $G$ with a dual complex group $\check{G}$, a \emph{Langlands parameter} is a $\check{G}$-conjugacy class of maps
%%\[
%%\phi: \Lfun_F \to \check{G},
%%\]
%%where $\Lfun_F$ is the conjectural Langlands group of the number field $F$.
%%An \emph{Arthur parameter} is a $\check{G}$-conjugacy class of maps
%%\[
%%\psi: \Lfun_F \times SL_2\bk{\C} \to \check{G} .
%%\]
%
%For a split group $G$ with a dual complex group $\check{G}$, an \emph{Arthur parameter} is a $\check{G}$-conjugacy class of maps
%\[
%\psi: \Lfun_F \times SL_2\bk{\C} \to \check{G} ,
%\]
%where $\Lfun_F$ is the conjectural Langlands group of the number field $F$, and such that
%\begin{itemize}
%	\item $\psi\bk{\Lfun_F}$ is bounded and contained in the set of semi-simple elements of $\check{G}$.
%	\item The restriction of $\psi$ to $SL_2\bk{\C}$ is algebraic.
%\end{itemize}
%
%
%Let $\phi:SL_2\bk{\C}\to\check{G}$ be given by $\phi\bk{g}=\psi\bk{1,g}$.
%The $\check{G}$-orbit of $im \phi$ is determined by $u=\phi\begin{pmatrix} 1&1\\0&1 \end{pmatrix}$.
%
%%Since $\psi\bk{\Lfun_F}$ is bounded and contains only semi-simple elements 	
%
%Since we are dealing only with residual representations whose cuspidal support lies along the torus, the map factors through $W_F\times SL_2\bk{\C}$, where $W_F$ is the Weil group of $F$.
%%
%%In fact, it factors through $W_{K/F}=W_F\rmod W_K$, where $K$ is a finite extension of $F$.
%%
%$\chi=\Id$ is the case where $\psi\bk{L_F}=1$.
%
%When $\chi\neq\Id$, the parameter $\psi$ factors through an endoscopic group $\check{L}$ of $\check{G}$
%\[
%\psi: L_F\times SL_2\bk{\C} \to \check{L} \hookrightarrow \check{G} 
%\]


%\begin{Rem}
%	Given a unipotent orbit $\mO$, the theory of nilpotent attaches to it a Jacobson-Morozov triple $\set{H,X,Y}$ and a labeled Dynkin diagram.
%	We recall that the labels $\epsilon_i$ on the nodes $\alpha_i$ satisfy $\epsilon_i = \gen{\alpha_i,H}$.
%	Here $\alpha_i$ should be a root of $\check{\bT}$.
%	Hence, the anti-dominant exponent of the associated spherical representation of $G\bk{F_v}$ is given by
%	\[
%	\mu = -\frac12\sum \epsilon_i \fun{i}
%	\]
%	We also note that a distinguished orbit is even and hence $\frac12\epsilon_i\in\set{0,1}$.
%	This is not true for a quasi-distinguished orbit.
%
%\end{Rem}






\section[Trivial $\chi$]{Unipotent Arthur Parameters for Degenerate Residual Representations of Groups of Type $E_n$ - Trivial $\chi$}

If $\chi=\Id$, \Cref{Eq:Satake_parameter_for_Arthur_parameter} implies that $\mu=\Id$, that is $\psi\res{\Lfun_F}=\Id$.
Hence, $\psi$ is determined by $X = \phi\begin{pmatrix} 1&1\\0&1 \end{pmatrix}$.
In other words, it is determined by the Satake parameter $\sigma_{\psi_v}$, which gives rise to the dominant weight $\lambda_{dom.} = \sigma_{\psi_v}$ of $T$.
That is, $\pi_{\Id_v}$ is the unique irreducible quotient of $i_{T\bk{F_v}}^{G\bk{F_v}}\lambda_{dom.}$.

It should be pointed out that, since we consider $\check{G}$-conjugacy classes of maps $\phi$, they are parameterized by distinguished nilpotent orbit $\check{G}$ and $\lambda_{dom.}$ can be read directly from the Weighted Dynkin diagrams.
More precisely, Given a unipotent orbit $\mO$, the theory of nilpotent attaches to it a Jacobson-Morozov triple $\gen{X, Y, H}$ and a labeled Dynkin diagram.
The semi-simple element $H=\phi\begin{pmatrix}q&\\&q^{-1}\end{pmatrix}$ is associated both with the weighted diagram and with $\sigma_{\psi_v}$.
By definition, the weight $\epsilon_i$ on the node $\alpha_i\in\Delta$, in the weighted Dynkin diagram, is given by $\epsilon_i = \gen{\alpha_i,H}$.
Thus, it holds that
\[
\lambda_{dom.} = \frac12\suml_{\alpha_i\in\Delta} \epsilon_i \fun{i} .
\]
Also, note that a distinguished orbit is even and hence $\epsilon_i\in\set{0,2}$.

Finally, before listing the various nilpotent orbits, irreducible square-integrable residual representations and Satake parameters, we recall a conjecture of Kim regarding which of the $\pi_{\eta_v}\in \Pi_{\psi_v}$ occurs in a principal series representation $i_{T\bk{F_v}}^{G\bk{F_v}} \lambda$.

\begin{Conj}[\cite{MR1426903}]
	If $\psi:SL_2\bk{\C}\to\check{G}$ is an Arthur parameter such that $\Pi_\psi$ contains a residual representation of $G$, then
	\begin{itemize}
		\item $\psi$ is associated to a distinguished orbit $\mO$ of $\check{G}$.
		\item Let $\Pi{\psi_v}^{res.}\subseteq \Pi_{\psi_v}$ consist of those representations which occur as local constituents of irreducible residual representations in the residual spectrum attached to the trivial character of $T\bk{\AA}\rmod T\bk{F}$.
		Then, $\Pi_{\psi_v}^{res.}$ is the image of $Springer\bk{\mO}$ under \Cref{Eq:Local_Arthur_cor}.
		Here, $Springer\bk{\mO}$ is the image of the Springer correspondence as described in \cite[\S 13.3]{MR1266626}.
	\end{itemize} 
\end{Conj}

Bellow, we list the various orbits which contribute to $L^2\bk{G}_{\coset{T,\Id}}$ and for each one, we also list $\Card{Springer\bk{\mO}}$ and $\Card{\Pi_{\psi_v}^{res.}}$.

\subsection{Case of $E_6$}

For the group of type $E_6$, we list the distinguished nilpotent orbits in $\check{E_6}$, the associated Satake parameter and data $\bk{i,s_0}$ such that $\ResRep{E_6}{i}{s_0}{\Id}$ realizes parts of $L^2_\psi$.
We also list the type of the component group $S_\psi$ as well as the cardinality of the image of the Springer correspondence and the that of $\Pi_{\psi_v}^{res.}$.

\begin{center}
	\begin{longtable}[h]{|c|c|c|c|c|c|}
		%	\begin{longtable}[H]{|c|c|c|c|}
			\hline
			Orbit & $\lambda_{dom.}$ & $\bk{i,s_0}$ & $S_\psi$ & $\Card{Sp\bk{\mO}}$ & $\Card{\Pi_{\psi_v}^{res.}}$
			\\ \hline \endhead \hline
			$E_6$ & $\esixchar{1}{1}{1}{1}{1}{1}$ & 
			\begin{tabular}{c}
				$\bk{1,6}$, $\bk{2,\frac{11}{2}}$, $\bk{3,\frac92}$, \\ $\bk{4,\frac72}$, $\bk{5,\frac92}$, $\bk{6,6}$
			\end{tabular}
			& 1 & 1 & 1 \\ \hline
			$E_6\bk{a_1}$ & $\esixchar{1}{1}{1}{0}{1}{1}$ & $\bk{1,3}$, $\bk{2,\frac72}$, $\bk{4,\frac52}$, $\bk{6,3}$ & 1 & 1 & 1 \\ \hline
			$E_6\bk{a_3}$ & $\esixchar{1}{0}{0}{1}{0}{1}$ & $\bk{2,\frac12}$, $\bk{3,\frac32}$, $\bk{4,\frac32}$, $\bk{5,\frac32}$ & $S_2$ & 2 & 1 \\ \hline
	\end{longtable}
	\label{Table:E6_Arthur}
\end{center}

\begin{itemize}
	\item The residual representation associated with the orbit $E_6$ is the trivial one.
	This residue is irreducible, in accordance with Arthur's conjectures.
	\item The residual representation associated with the orbit $E_6\bk{a_1}$ is the minimal one.
	This residue is irreducible, in accordance with Arthur's conjectures.
	\item The residual representation associated with the orbit $E_6\bk{a_3}$ is irreducible.
	According to Arthur's conjectures, the local packet $\Pi_{\psi_v} = \set{\pi_{1,v}, \pi_{sgn,v}}$ contains two irreducible representations.
	By \Cref{Eq:Arthurs_multiplicity_formula}, both will appear in the discrete spectrum.
	Indeed, for a finite subset $S\subset\Places$, let $\eta_S=\otimes_{v\in S} \sgn_v \otimes_{v\notin S} \Id_v$.
	Then,
	\[
	m_\eta = \piece{0, & \Card{S}\equiv 1 \pmod{2} \\ 
		1, & \Card{S}\equiv 0 \pmod{2}} .
	\]
	However, only $S_\emptyset$ appears in the degenerate principal series.
	By Kim's conjecture, the other $\pi_{\eta_S}$ will appear in the residual spectrum, but only as residues of Eisenstein series induced from smaller parabolic subgroups.
\end{itemize}

Note that, as opposed to the following cases, the next to minimal representation does not appear here.
This has to do with the fact that the next-to-minimal nilpotent orbit, $D_5$, is not distinguished (or even quasi-distinguished) and the next-to-minimal residual representation is not square-integrable.


\subsection{Case of $E_7$}

\begin{center}
	\begin{longtable}[h]{|c|c|c|c|c|c|}
	%	\begin{longtable}[H]{|c|c|c|c|}
		\hline
		Orbit & $\lambda_{dom.}$ & $\bk{i,s_0}$ & $S_\psi$ & $\Card{Sp\bk{\mO}}$ & $\Card{\Pi_{\psi_v}^{res.}}$
		\\ \hline \endhead \hline
		$E_7$ & $\esevenchar{1}{1}{1}{1}{1}{1}{1}$ & 
		\begin{tabular}{c}
			$\bk{1,\frac{17}{2}}$, $\bk{2,7}$, $\bk{3,\frac{11}{2}}$, $\bk{4,4}$, \\
			$\bk{5,5}$, $\bk{6,\frac{13}{2}}$, $\bk{7,9}$
		\end{tabular}
		 & 1 & 1 & 1 \\ \hline
		$E_7\bk{a_1}$ & $\esevenchar{1}{1}{1}{0}{1}{1}{1}$
		& $\bk{1,\frac{11}{2}}$, $\bk{2,5}$, $\bk{4,3}$, $\bk{7,5}$ & 1 & 1 & 1 \\ \hline
		$E_7\bk{a_2}$ & $\esevenchar{1}{1}{1}{0}{1}{0}{1}$
		& $\bk{1,\frac72}$, $\bk{5,3}$, $\bk{6,\frac72}$, $\bk{7,1}$ & 1 & 1 & 1 \\ \hline
		$E_7\bk{a_3}$ & $\esevenchar{1}{0}{0}{1}{0}{1}{1}$
		& $\bk{1,\frac12}$, $\bk{3,\frac52}$, $\bk{4,2}$, $\bk{6,\frac52}$ & $S_2$ & 2 & 1 \\ \hline
		$E_7\bk{a_4}$ & $\esevenchar{1}{0}{0}{1}{0}{0}{1}$
		& $\bk{3,\frac32}^\ast$, $\bk{6,\frac12}^\ast$, $\bk{2,1}$ & $S_2$ & 2 & 2 \\ \hline
		$E_7\bk{a_5}$ &  $\esevenchar{0}{0}{0}{1}{0}{0}{1}$
		& $\bk{3,\frac12}$, $\bk{4,1}$, $\bk{5,1}$ & $S_3$ & 3 & 1 \\ \hline
	\end{longtable}
	\label{Table:E7_Arthur}
\end{center}


\begin{itemize}
	\item The residual representation associated with the orbit $E_7$ is the trivial one.
	This residue is irreducible, in accordance with Arthur's conjectures.
	\item The residual representation associated with the orbit $E_7\bk{a_1}$ is the minimal one.
	This residue is irreducible, in accordance with Arthur's conjectures.
	\item The residual representation associated with the orbit $E_7\bk{a_2}$ is the next-to-minimal one.
	This residue is irreducible, in accordance with Arthur's conjectures.
	\item In the case of the orbit $E_7\bk{a_3}$, one can carry an analysis similar to that of the orbit $E_6\bk{a_3}$ of $E_6$.
	\item The residual representation associated with the orbit $E_7\bk{a_4}$ is not irreducible, while the residual representations at $\bk{3,\frac32}$ and $\bk{6,\frac12}$ are.
	By Arthur's conjecture, the local packets $\Pi_{\psi_v}=\set{\pi_{1,v}, \pi_{\sgn,v}}$ should consist of two irreducible representation and by Kim's conjecture, both should appear in the residual spectrum.
	Together with the multiplicities
	\[
	m_\eta = \piece{0, & \Card{S}\equiv 1 \pmod{2} \\ 
		1, & \Card{S}\equiv 0 \pmod{2}} ,
	\]
	where $\eta_S=\otimes_{v\in S} \sgn_v \otimes_{v\notin S} \Id_v$.
	Indeed, that has been proved to be the case in \Cref{Prop:Residue_E7_2_1_1}. That is, $L^2_\psi\ResRep{E_6}{2}{1}{\Id}$.
	In particular, the eigenvalue calculated in \Cref{Appendix:Local_data_for_global_SI_resisudes} could be inferred from the multiplicity formula.
	
	We point out that $\ResRep{E_6}{3}{\frac32}{\Id}$ $\ResRep{E_6}{6}{\frac12}{\Id}$ only realize $\pi_{\Id}$.

	\item The residual representation associated with the orbit $E_7\bk{a_5}$ is irreducible.
	However, here $S_\psi=S_3$ and Arthur's and Kim's conjectures expect that $\Pi_{\psi_v}=\set{\pi_{\Id,v}, \pi_{\sgn,v}, \pi_{\tau,v}}$.
	Here, $\tau$ denotes the irreducible $2$-dimensional representation of $S_3$.
	For $\dot{S}=S_{\sgn}\cupdot S_\tau$, write
	\[
	\eta_{\dot{S}} = \otimes_{v\notin \dot{S}} \Id_v \otimes_{v\in S_{\sgn}} \sgn_v \otimes_{v\in S_\tau} \tau_v.
	\]
	Then, the expected multiplicity of $\eta_{\dot{S}}$ in $L^2_{dis.}$ is
	\[
	m_{\eta_{\dot{S}}} = \piece{
	0, & \Card{S_\tau}=0,\ \Card{S_{\sgn}}\equiv 1 \pmod{2} \\
	1, & \Card{S_\tau}=0,\ \Card{S_{\sgn}}\equiv 0 \pmod{2} \\
	0, & \Card{S_\tau} = 1 \\
	\frac{2^{\Card{S_{\tau}}}+2\cdot\bk{-1}^{\Card{S_{\tau}}}}{6}, & \Card{S_{\tau}} > 1 . }
	\]
	It is interesting to point out that for $\Card{S_\tau}>1$, the multiplicities $m_\eta$ forms an unbounded sequence of numbers.
	Such a sequence is known to occur in the cuspidal spectrum of $G_2$ (see \cite{MR2192822,MR1918673} for more information).
\end{itemize}



\subsection{Case of $E_8$}

\begin{center}
	\begin{longtable}[h]{|c|c|c|c|c|c|}
		%	\begin{longtable}[H]{|c|c|c|c|}
		\hline
		Orbit & $\lambda_{dom.}$ & $\bk{i,s_0}$ & $S_\psi$ & $\Card{Sp\bk{\mO}}$ & $\Card{\Pi_{\psi_v}^{res.}}$
		\\ \hline \endhead \hline
		$E_8$ & $\eeightchar{1}{1}{1}{1}{1}{1}{1}{1}$ & 
		\begin{tabular}{c}
			$\bk{1,\frac{23}{2}}$, $\bk{2,\frac{17}{2}}$, $\bk{3,\frac{13}{2}}$, $\bk{4,\frac{9}{2}}$, \\ $\bk{5,\frac{11}{2}}$, $\bk{6,7}$, $\bk{7,\frac{19}{2}}$, $\bk{8,\frac{29}{2}}$
		\end{tabular}
		& 1 & 1 & 1 \\ \hline
		$E_8\bk{a_1}$ & $\eeightchar{1}{1}{1}{0}{1}{1}{1}{1}$ 
		& $\bk{1,\frac{17}{2}}$, $\bk{2,\frac{13}{2}}$, $\bk{4,\frac72}$, $\bk{8,\frac{19}{2}}$
		& 1 & 1 & 1 \\ \hline
		$E_8\bk{a_2}$ & $\eeightchar{1}{1}{1}{0}{1}{0}{1}{1}$ 
		& $\bk{1,\frac{13}{2}}$, $\bk{5,\frac{7}{2}}$, $\bk{7,\frac{11}{2}}$, $\bk{8,\frac{11}{2}}$
		& 1 & 1 & 1 \\ \hline
		$E_8\bk{a_3}$ & $\eeightchar{1}{0}{0}{1}{0}{1}{1}{1}$ 
		& $\bk{3,\frac72}$, $\bk{4,\frac52}$, $\bk{7,\frac92}$, $\bk{8,\frac12}$
		& $S_2$ & 2 & 1 \\ \hline
		$E_8\bk{a_4}$ & $\eeightchar{1}{0}{0}{1}{0}{1}{0}{1}$ & $\bk{1,\frac72}$, $\bk{2,\frac72}$, $\bk{5,\frac52}$, $\bk{6,3}$
		& $S_2$ & 2 & 1 \\ \hline
		$E_8\bk{b_4}$ & $\eeightchar{1}{0}{0}{1}{0}{0}{1}{1}$ & $\bk{3,\frac52}^\ast$, $\bk{7,\frac52}^\ast$, $\bk{1,\frac52}$
		& $S_2$ & 2 & 2 \\ \hline
		$E_8\bk{a_5}$ & $\eeightchar{1}{0}{0}{1}{0}{0}{1}{0}$ & $\bk{1,\frac12}^\ast$, $\bk{2,\frac52}^\ast$, $\bk{7,\frac32}$
		& $S_2$ & 2 & 2 \\ \hline
		$E_8\bk{b_5}$ & $\eeightchar{0}{0}{0}{1}{0}{0}{1}{1}$ & $\bk{4,\frac32}$, $\bk{6,2}$, $\bk{7,\frac12}$
		& $S_3$ & 3 & 1 \\ \hline
		$E_8\bk{a_6}$ & $\eeightchar{0}{0}{0}{1}{0}{0}{1}{0}$ & $\bk{2,\frac32}$, $\bk{3,\frac32}$, $\bk{5,\frac32}$
		& $S_3$ & 3 & 1 \\ \hline
		$E_8\bk{b_6}$ & $\eeightchar{0}{0}{0}{1}{0}{0}{0}{1}$ & $\bk{2,\frac12}^{?}$, $\bk{6,1}$
		& $S_3$ & 3 & ? \\ \hline
		$E_8\bk{a_7}$ & $\eeightchar{0}{0}{0}{0}{1}{0}{0}{0}$ & $\bk{4,\frac12}$, $\bk{5,\frac12}^{?}$
		& $S_5$ & 6 & ? \\ \hline
	\end{longtable}
	\label{Table:E8_Arthur}
\end{center}

\begin{itemize}
	\item The residual representation associated with the orbit $E_8$ is the trivial one.
	This residue is irreducible, in accordance with Arthur's conjectures.
	\item The residual representation associated with the orbit $E_8\bk{a_1}$ is the minimal one.
	This residue is irreducible, in accordance with Arthur's conjectures.
	\item The residual representation associated with the orbit $E_8\bk{a_2}$ is the next-to-minimal one.
	This residue is irreducible, in accordance with Arthur's conjectures.
	\item In the cases of the orbits $E_8\bk{a_3}$ and $E_8\bk{a_4}$, one can carry an analysis similar to that of the orbit $E_6\bk{a_3}$ of $E_6$.
	\item In the cases of the orbits $E_8\bk{b_4}$ and $E_8\bk{a_5}$, one can carry an analysis similar to that of the orbit $E_7\bk{a_4}$ of $E_7$.
	\item In the cases of the orbits $E_8\bk{b_5}$ and $E_8\bk{a_6}$, one can carry an analysis similar to that of the orbit $E_7\bk{a_5}$ of $E_7$.
%	\item The residual representation associated with the orbit $E_8\bk{a_4}$ is...
%	\item The residual representation associated with the orbit $E_8\bk{b_4}$ is not irreducible... However, the residual representations at $\bk{3,\frac52}$ and $\bk{7,\frac52}$ are...
%	\item The residual representation associated with the orbit $E_8\bk{a_5}$ is not irreducible... However, the residual representations at $\bk{1,\frac12}$ and $\bk{2,\frac52}$ are...
%	\item The residual representation associated with the orbit $E_8\bk{b_5}$ is...
%	\item The residual representation associated with the orbit $E_8\bk{a_6}$ is...
	\item The residual representation associated with the orbit $E_8\bk{b_6}$ is...???
	\item The residual representation associated with the orbit $E_8\bk{a_7}$ is...???
	\todonum{Complete the last two parts in accordance to the local results.}
\end{itemize}


\begin{Rem}
	One of the conclusions of the discussion above, is that for each square-integrable residual representation $\pi$ of $G$ of type $E_n$, Kim's conjecture anticipates that it appears in $L^2_{res}\bk{G\bk{\AA}\rmod G\bk{F}}$ with multiplicity $1$.
	\todonum{This is not we want to say here. We want to talk about representations which do not intersect the residual spectrum at all or to say that we expect that the multiplicity of other representations is at most 1 in the residual spectrum, but this has nothing to do with Arthur's or Kim's conjectures.}
	Hence, $\pi$ is not expected to have an embedding into the cuspidal spectrum.
	
	It should be noted that such representations do exist for groups such as $SL_n$ (see \cite{MR1303497}) and $SO_{2n}$, for which the Dynkin diagram admits a non-trivial outer automorphism. Thus, one could have expected for such an example to occur for $G$ of type $E_6$.
	\todonum{Maybe there is such an example if we take the outer automorphism into account somehow?}
	We also note that another such example occurs for $G_2$ (see \cite{MR2192822}).
\end{Rem}



%Multiplicity formulas
%
%
%\begin{center}
%	\begin{longtable}[h]{|c|c|}
%%	\begin{longtable}[H]{|c|c|c|c|}
%		\hline
%		$S_\psi$ & $m\bk{\pi_S}$
%		\\ \hline \endhead \hline
%		$1$ & $1$ \\ \hline
%		$S_2$ & $1$ \\ \hline
%	\end{longtable}
%	\label{Table:Multiplicities}
%\end{center}


\section[Non-trivial $\chi$]{Unipotent Arthur Parameters for Degenerate Residual Representations of Groups of Type $E_n$ - Non-trivial $\chi$}

An endoscopic group $H$ of $G$ is, roughly speaking, a quasi-split group such that $\ldual{H} = Cent\bk{s, \ldual{G}}^0$ for some semi-simple element $s\in\ldual{G}$.
Since we are dealing with split connected groups, we may replace replace $\ldual{G}$ and $\ldual{H}$ with $\check{G}$ and $\check{H}$ in the definition.

For a square-integrable residue $\ResRep{G}{i}{s_0}{\chi}$, with $\chi\neq\Id$, we expect that the corresponding Arthur parameter $\psi$ will factor through $\check{H}$ for some endoscopic group $H$ of $G$.
\[
\xymatrix{
	\psi: W_F \times SL_2\bk{\C} \ar[dr]_{\psi'=\bk{\phi',\mu'}}  \ar[rr] & & \check{G} \\
	& \check{H} \ar[ur] & 
}
\]
In particular, we expect this to happen in such a way that $\phi'$ corresponds to the principal unipotent orbit of $\check{H}$.

Therefore, in order to describe the parameter $\psi$, it is enough to describe the map to $\check{H}$ and the embedding $\check{H}\hookrightarrow\check{G}$.
The latter is given by various works such as \cite{MR32659,MR294349,MR2044850,MR1048074,MR1264015}.
\redcolor{We actually care more about pseudo-Levi subgroups as in Sommers' paper}
In order to describe the former, we will proceed as follows:
\begin{itemize}
	\item To a residual representations $\ResRep{G}{i}{s_0}{\chi}$ we will associate a nilpotent orbit $\mO_G$ of $\check{G}$ using the Satake parameter at unramified places and \Cref{Eq:Satake_parameter_for_Arthur_parameter}.
	
	\item To $\mO_G$ we will associate an endoscopic group $H$ of $G$ by fixing its complex dual $\check{H}$ so that $\mO_G$ is the $\check{G}$-saturation of the principal orbit of $\check{H}$.
	For most cases, this can be done using \cite{MR2526390} (note that, in our case, $p=\infty$).
%	We also attach a nilpotent orbit, usually the principal one, $\mO_H$ of $\check{H}$.
%	This is done using the data in \cite{MR2526390} (note that here, $p=\infty$).
	
	\item We then describe the parameter $\psi$ using the induced map $W_F \times SL_2\bk{\C}\to \check{H}$.
	
\end{itemize}


It is useful to recall that maximal subgroups of $\check{G}$, which contain a maximal torus, could be read from the extended Dynkin diagram using the Borel-de Siebenthal theory (see \cite{MR32659}).
This is the diagram attained by adding the negative highest root $\alpha_0$ of $\check{G}$ to the usual Dynkin diagram.
The added root $\alpha_0$ is given by
\[
\alpha_0 = \piece{-\fun{2}, & G=E_6 \\ -\fun{1}, & G=E_7 \\ -\fun{8}, & G=E_8 .}
\]
The extended Dynkin diagrams of the various $E_n$ will be given bellow.

In what follows, 

%\redcolor{Maybe it is worth mentioning that the reductive part of the centralizer of a unipotent orbit, comprises of a connected part which is a semi-simple group (in cases which interest us) and a component group (semi-direct product).
%Assuming that the orbit is a saturation of a principal orbit of a closed subgroup $H$ attained by removing nodes from the extended Dynkin diagram, than the component group is the automorphism group of the Dynkin diagram of $H$}


\subsection{Case of $E_6$}

Recall the extended Dynkin diagram of type $E_6$:
\[\begin{tikzpicture}[scale=0.5]
	\draw (-1,0) node[anchor=east]{};
	\draw (0 cm,0) -- (8 cm,0);
	\draw (4 cm, 0 cm) -- +(0,4 cm);
	\draw[fill=black] (0 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_1$};
	\draw[fill=black] (2 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_3$};
	\draw[fill=black] (4 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_4$};
	\draw[fill=black] (6 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_5$};
	\draw[fill=black] (8 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_6$};
	\draw[fill=black] (4 cm, 2 cm) circle (.25cm) node[right=3pt]{$\alpha_2$};
	\draw[fill=black] (4 cm, 4 cm) circle (.25cm) node[right=3pt]{$\alpha_0$};
\end{tikzpicture}\]

The proper maximal cuspidal endoscopic groups $H$ of $E_6$ have a complex dual $\check{H}$ of type $A_5\times A_1$ and $A_2\times A_2\times A_2$, these can be attained by removing the roots $\alpha_2$ and $\alpha_4$ (respectively) from the extended Dynkin diagram.

\begin{center}
	\begin{longtable}[h]{|c|c|c|c|}
%	\begin{longtable}[H]{|c|c|c|c|}
		\hline
		$Type\bk{\check{H}}$ & $\check{H}$ & $\cZ\bk{\check{H}}$ & $Out\bk{\check{H}}$
		\\ \hline \endhead \hline
%		$A_5\times A_1$ & $PGL_6\bk{\C} \times PGL_2\bk{\C}$ & 1 & $S_2$  \\ \hline
		$A_5\times A_1$ & $\bk{SL_6\bk{\C}\rmod \mu_3 \times SL_2\bk{\C}}\rmod \mu_2$ & $\mu_2$ & $S_2$ \\ \hline
%		$A_2\times A_2\times A_2$ & $\bk{SL_3\bk{\C}\rmod \mu_3}\times \bk{SL_3\bk{\C}\rmod \mu_3} \times SL_3\bk{\C}$ & $\mu_3$ \\ \hline
		$A_2\times A_2\times A_2$ & $\bk{SL_3\bk{\C}}^3\rmod \mu_3^2$ & $\mu_3$ & $S_3$ \\ \hline
	\end{longtable}
	\label{Table:E6_proper_maximal_cuspidal_endoscopic_groups}
\end{center}

In the following table, we sort the square-integrable residual representations $\ResRep{G}{i}{s_0}{\chi}$ with non-trivial $\chi$, sorted by their associated nilpotent orbit, together with the Satake parameter at unramified places.
Note that we write here $\chi$ for $\chi_v\bk{\unif_v}$.
We also list the complex dual $\check{H}$ of the associated endoscopic group.
In both cases, $\phi'$ is associated with the principal orbit in $\check{H}$.
Finally, 

\begin{center}
	\begin{longtable}[h]{|c|c|c|c|}
		%	\begin{longtable}[H]{|c|c|c|c|}
			\hline
			Orbit & $\sigma_{\psi_v}$ & $\bk{i,s_0,ord\bk{\chi}}$ & $Type\bk{\check{H}}$ 
			%		& $\Card{Sp\bk{\mO}}$
			\\ \hline \endhead \hline
			$E_6\bk{a_3}$ & $\esixchar{1}{\chi}{\chi}{1}{\chi}{1}$ & $\bk{2,\frac12,2}$, $\bk{3,\frac32,2}$, $\bk{4,\frac32,2}$, $\bk{5,\frac32,2}$ & $A_5\times A_1$  \\ \hline
			%		& 2 \\ \hline
			$D_4\bk{a_1}$ & $\esixchar{\chi}{\chi}{\chi}{1}{\chi}{\chi}$ & $\bk{4,\frac12,3}$ & $A_2\times A_2\times A_2$ \\ \hline
			%		& 3 \\ \hline
		\end{longtable}
		\label{Table:E6_Arthur_Chi_Non-trivial}
	\end{center}

%\begin{center}
%	\begin{longtable}[h]{|c|c|c|c|c|}
%%	\begin{longtable}[H]{|c|c|c|c|}
%		\hline
%		Orbit & $\sigma_{\psi_v}$ & $\bk{i,s_0,ord\bk{\chi}}$ & $Type\bk{\check{H}}$ & $S_\psi$
%		%		& $\Card{Sp\bk{\mO}}$
%		\\ \hline \endhead \hline
%		$E_6\bk{a_3}$ & $\esixchar{1}{\chi}{\chi}{1}{\chi}{1}$ & $\bk{2,\frac12,2}$, $\bk{3,\frac32,2}$, $\bk{4,\frac32,2}$, $\bk{5,\frac32,2}$ & $A_5\times A_1$ & 1 \\ \hline
%		%		& 2 \\ \hline
%		$D_4\bk{a_1}$ & $\esixchar{\chi}{\chi}{\chi}{1}{\chi}{\chi}$ & $\bk{4,\frac12,3}$ & $A_2\times A_2\times A_2$ & $S_2$ \\ \hline
%		%		& 3 \\ \hline
%	\end{longtable}
%	\label{Table:E6_Arthur_Chi_Non-trivial}
%\end{center}

The data in this table should be read as follows:
\begin{itemize}
	\item The unipotent orbit $E_6\bk{a_3}$ of $E_6$ corresponds to the principal orbit $A_5\oplus A_1$ in $\check{H}=\bk{SL_6\bk{\C}\rmod \mu_3 \times SL_2\bk{\C}}\rmod \mu_2$ of type $A_5\times A_1$.
	It holds that $S_\phi=\cZ\bk{\check{H}} = \cZ\bk{SL_6\bk{\C}\rmod \mu_3} \cong \mu_2$.
	Thus, for a quadratic Hecke character $\chi$, we take $\psi$ to be
	\[
	\psi\bk{w,g} 
	= \bk{ \chi\bk{w}\Id_6, \Id_2 } \phi\bk{g}
	\]
	Hence, $\widehat{S_\psi} = \set{1}$.
	Furthermore, taking $\eta=\Id$, \Cref{Eq:Arthurs_multiplicity_formula} implies that $m_\eta=1$ and hence
	\[
	\begin{split}
		L^2_\psi
		& = \ResRep{E_6}{2}{\frac12}{\chi} 
		= \ResRep{E_6}{3}{\frac32}{\chi} \\
		& = \ResRep{E_6}{4}{\frac32}{\chi} 
		= \ResRep{E_6}{5}{\frac32}{\chi}.
	\end{split}
	\]
	
	\todonum{It seems like $S_\psi$ should be $S_2$}
		
	\item Note that the orbit $D_4\bk{a_1}$ of $E_6$ is not distinguished but it is quasi-distinguished, even and special.
	By \cite[pg. 402]{MR1266626}, we have $C_\phi^0$ is a 2-dimensional torus and the component group of the centralizer is $C_\phi\rmod C_\phi^0 \cong S_3$.
	This orbit corresponds to the principal orbit $A_2\oplus A_2\oplus A_2$ in $A_2\times A_2\times A_2$.
	Hence, the corresponding parameters will factor through $\check{H}=\bk{SGL_3\bk{\C}}^3\rmod \mu_3^2$.
	Thus, for a cubic Hecke character $\chi$, we take $\psi$ to be
	\[
	\psi\bk{w,g} 
	 = \bk{\coset{\begin{matrix}\chi\bk{w}&&\\&\chi\bk{w}&\\&&\chi\bk{w} \end{matrix}}, \coset{\begin{matrix}\chi\bk{w}&&\\&\chi\bk{w}&\\&&\chi\bk{w} \end{matrix}},\coset{\begin{matrix}\chi\bk{w}&&\\&\chi\bk{w}&\\&&\chi\bk{w}\end{matrix}}} \phi\bk{g}
	\]
	Hence, $C_\psi\rmod C_\psi^0 \cong \mu_3$.
	This implies that:
	\begin{itemize}
		\item For a place $v$ such that $\chi_v\neq\Id_v$, it holds that $\Pi_{\psi_v}=\set{\pi_{\Id,v}, \pi_{\kappa,v}, \pi_{\kappa^2,v}}s$, where $\set{\Id, \kappa, \kappa^2}$ are the three irreducible representations of $\mu_3$.
		\item For a place where $\chi_v=\Id_v$, it holds that $S_\psi \cong S_3$ and $\Pi_{\psi_v}=\set{\pi_{\Id,v}, \pi_{\sgn,v}, \pi_{\tau,v}}$.
		In the degenerate residual spectrum we encounter only $\pi_{\Id,v}$ though.
	\end{itemize}
	Let $S_\kappa$ denote the places where $\chi_v\neq\Id_v$ and $\eta_v=\kappa$ and let $S_{\kappa^2}$ denote the places where $\chi_v\neq\Id_v$ and $\eta_v=\kappa^2$.	
	The multiplicity formula \Cref{Eq:Arthurs_multiplicity_formula} then yields
	\[
	m_\eta = \piece{1,& \Card{S_\kappa}\equiv \Card{S_{\kappa^2}}\pmod{3} \\ 0,& \Card{S_\kappa}\not\equiv \Card{S_{\kappa^2}}\pmod{3},}
	\]
	which is consistent with \Cref{Prop:E6_4_1-2_3_Residue}.
	In particular,
	\[
	L^2_\psi
	= \ResRep{E_6}{4}{\frac12}{\chi} .
	\]
	
%Stab=
%[1, w2*w4*w5*w6*w3*w4*w5*w1*w3*w4*w2, w6*w5*w4*w3*w2*w4*w5*w6*w1*w3*w4*w5*w2*w4*w3*w1, w1*w3*w4*w5*w6*w2*w4*w5*w3*w4*w1*w3*w2*w4*w5*w6, w5*w6*w4*w5*w3*w4*w1*w3*w2*w4*w5*w6*w3*w4*w1*w3*w2*w4*w5, w3*w4*w1*w3*w2*w4*w5*w6*w4*w3*w2*w4*w5*w4*w3*w2*w4*w1*w3]
%Stab[1]*Stab[1]==1
%Stab[2]*Stab[2]==Stab[3]
%Stab[1]*Stab[2]==Stab[5]
%Stab[4]*Stab[1]==Stab[2]
%Stab[2]*Stab[2]*Stab[2]==1
%w=Stab[2]
%sage: for ch in L:
%....:     print(E6.coordinate_vector_of_char(ch,'roots'),E6.coordinate_vector_of_char(w.action(ch),'roots'))
%....:
%[1, 0, 0, 0, 0, 0] [-1, -2, -2, -3, -2, -1]
%[0, 1, 0, 0, 0, 0] [0, 0, 0, 0, 1, 0]
%[0, 0, 1, 0, 0, 0] [0, 1, 0, 0, 0, 0]
%[0, 0, 0, 0, 1, 0] [0, 0, 1, 0, 0, 0]
%[0, 0, 0, 0, 0, 1] [1, 0, 0, 0, 0, 0]
%[-1, -2, -2, -3, -2, -1] [0, 0, 0, 0, 0, 1]
%sage: s=Stab[1]
%sage: for ch in L:
%....:     print(E6.coordinate_vector_of_char(ch,'roots'),E6.coordinate_vector_of_char(s.action(ch),'roots'))
%....:
%[1, 0, 0, 0, 0, 0] [0, 0, 0, 0, 1, 0]
%[0, 1, 0, 0, 0, 0] [-1, -2, -2, -3, -2, -1]
%[0, 0, 1, 0, 0, 0] [0, 0, 0, 0, 0, 1]
%[0, 0, 0, 0, 1, 0] [1, 0, 0, 0, 0, 0]
%[0, 0, 0, 0, 0, 1] [0, 0, 1, 0, 0, 0]
%[-1, -2, -2, -3, -2, -1] [0, 1, 0, 0, 0, 0]

%%%%%%%
%%%w:
% e_1->e_0, e_3->e_2
% e_0->e_6, e_2->e_5
% e_5->e_3, e_6->e_1

%%%s:
% e_1->e_5, e_3->e_6
% e_2->e_0, e_0->e_2
% e_5->e_1, e_6->e_3


	
	
\end{itemize}





%\sepline
%
%
%
%\begin{itemize}
%	\item The unipotent orbit $E_6\bk{a_3}$ corresponds to the principal orbit $A_5\oplus A_1$ in $\check{H}$ of type $A_5\times A_1$.
%	The center of $\check{H}$ is $\mu_2$ and hence, a parameter $\psi$ of $G$, which factors through $\check{H}$, gives rise to a map $\mu:W_F \to \mu_2$.
%	By class field theory, $\mu$ corresponds to a quadratic Hecke character $\chi$ of $\AA^\times$.
%	In turn, the embedding $\check{H}\hookrightarrow \check{G}$ then yields the Satake parameter given in the table.
%	
%	$S_\psi = S_\varphi\rmod \cZ\bk{H} = S_2\rmod\mu_2 \cong 1$
%	
%	We thus conclude that
%	\[
%	L^2_\psi
%	= \ResRep{E_6}{2}{\frac12}{\chi}
%	= \ResRep{E_6}{3}{\frac32}{\chi}
%	= \ResRep{E_6}{4}{\frac32}{\chi}
%	= \ResRep{E_6}{5}{\frac32}{\chi} .
%	\]
%	
%	\item Dealing with the unipotent orbit, we first note that $D_4\bk{a_1}$ is not distinguished but it is quasi-distinguished, even and special.
%	This orbit corresponds to the principal orbit $A_2\oplus A_2\oplus A_2$ in $A_2\times A_2\times A_2$.
%	The center of $\check{H}$ is $\mu_3$ and, as above, a parameter $\psi$ which factors through $\check{H}$ will give rise to a cubic Hecke character $\chi$ of $\AA^\times$.
%	It thus follows that $S_\psi = S_\varphi\rmod \cZ\bk{H} = S_3\rmod\mu_3 \cong S_2$
%	
%	\[
%	L^2_\psi
%	= \ResRep{E_6}{4}{\frac12}{\chi} .
%	\]
%\end{itemize}
%
%
%\sepline

%\begin{center}
%\begin{longtable}[h]{|c|c|c|c|}
%	%	\begin{longtable}[H]{|c|c|c|c|}
%		\hline
%		Orbit & $\Real\bk{\lambda_{dom.}}$ & $\bk{i,s_0,ord\bk{\chi}}$ & Comp  
%%		& $\Card{Sp\bk{\mO}}$
%		\\ \hline \endhead \hline
%		$E_6\bk{a_3}$ & $\esixchar{1}{0}{0}{1}{0}{1}$ & $\bk{2,\frac12,2}$, $\bk{3,\frac32,2}$, $\bk{4,\frac32,2}$, $\bk{5,\frac32,2}$ & $S_2$ \\ \hline
%%		& 2 \\ \hline
%		$D_4\bk{a_1}$ & $\esixchar{0}{0}{0}{1}{0}{0}$ & $\bk{4,\frac12,3}$ & $S_3$ \\ \hline
%%		& 3 \\ \hline
%	\end{longtable}
%%	\label{Table:E6_Arthur_Chi_Non-trivial}
%\end{center}
%$D_4\bk{a_1}$ is not distinguished but it is quasi-distinguished, even and special.
%Also, it should be noted that all of $\bk{2,\frac12,2}$, $\bk{3,\frac32,2}$, $\bk{4,\frac32,2}$, $\bk{5,\frac32,2}$ are in the same orbit.
%\todonum{Explain or change the phrasing "in the same orbit"}
%Furthermore, let
%\[
%%\mu_v\bk{Fr_v} = \esixchar{\chi}{\chi}{\chi}{\chi}{\chi}{\chi}
%\mu_v\bk{Fr_v} = \esixchar{0}{\chi}{\chi}{0}{\chi}{0}
%\]
%
%
%
%\[
%\psi\bk{Fr_v,\begin{pmatrix}q^{\frac12} & \\ & 1^{-\frac12} \end{pmatrix}}
%= \piece{\esixchar{1}{\chi}{\chi}{1}{\chi}{1}, & E_6\bk{a_3} \\ 
%\esixchar{\chi}{\chi}{\chi}{1}{\chi}{\chi}, & D_4\bk{a_1}} .
%\]
%\redcolor{In both cases, this is the correct description of $\mu$, but for different $\chi$. Note that $\chi_v$ is, in itself, defined by a map $\mu_{\chi_v}:W_{F_v} \to \C\times $.}

%\begin{center}
%	\begin{longtable}[h]{|c|c|c|c|}
%%	\begin{longtable}[H]{|c|c|c|c|}
%		\hline
%		$C_G$ & $H$ & $C_H$ & Principal
%		%		& $\Card{Sp\bk{\mO}}$
%		\\ \hline \endhead \hline
%		$E_6\bk{a_3}$ & $A_5\times A_1$ & $A_5\oplus A_1$ & \cmark \\ \hline
%		$D_4\bk{a_1}$ & $A_2\times A_2\times A_2$ & $A_2\oplus A_2\oplus A_2$ & \cmark \\ \hline
%%		$D_4\bk{a_1}$ & $C_4$ & $A_1\oplus C_2$ & \xmark \\ \hline
%%		$D_4\bk{a_1}$ & $A_5\times A_1$ & $A_3+A_1\oplus A_1$ & \xmark \\ \hline
%	\end{longtable}
%	\label{Table:E6_Orbits_and_Endoscopy}
%\end{center}

%\redcolor{Note that $E_6\bk{a_1}$ also correspond to the principal orbit of $G_2$ and $C_4$, while $E_6\bk{a_3}$ correspond to that of $A_2$. Can we make predictions regarding those? Do they appear in the square-integrable spectrum?}

\subsection{Case of $E_7$}

The extended Dynkin diagram of type $E_7$ is 
\[\begin{tikzpicture}[scale=0.5]
	\draw (-1,0) node[anchor=east]{};
	\draw (-2 cm,0) -- (10 cm,0);
	\draw (4 cm, 0 cm) -- +(0,2 cm);
	\draw[fill=black] (0 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_1$};
	\draw[fill=black] (2 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_3$};
	\draw[fill=black] (4 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_4$};
	\draw[fill=black] (6 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_5$};
	\draw[fill=black] (8 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_6$};
	\draw[fill=black] (10 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_7$};
	\draw[fill=black] (4 cm, 2 cm) circle (.25cm) node[right=3pt]{$\alpha_2$};
	\draw[fill=black] (-2 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_0$};
\end{tikzpicture}\]

The proper maximal cuspidal endoscopic groups $H$ of $E_7$ have a complex dual $\check{H}$ of type $D_6\times A_1$, $A_7$ and $A_5\times A_2$, these can be attained by removing the roots $\alpha_1$, $\alpha_2$ and $\alpha_3$ (respectively) from the extended Dynkin diagram.
The group $E_7$ also admits endoscopic groups $H$ with $\check{H}$ of type $A_1\times A_1$ and $G_2\times A_1$, these are maximal among subgroups not containing a maximal torus.

\begin{center}
	\begin{longtable}[h]{|c|c|c|c|}
		\hline
		$Type\bk{\check{H}}$ & $\check{H}$ & $\cZ\bk{\check{H}}$ & $Out\bk{\check{H}}$
		\\ \hline \endhead \hline
		$D_6\times A_1$ & $\coset{\bk{Spin_{12}\bk{\C}\rmod \mu_2}\times SL_2\bk{\C}}\rmod \mu_2$ & $\mu_2$ & $S_2$ \\ \hline
		$A_7$ & $SL_8\bk{\C}\rmod \mu_4$ & $\mu_2$ & $S_2$ \\ \hline
		$A_5\times A_2$ & $\bk{\bk{SL_6\bk{\C}\rmod \mu_2} \times SL_3\bk{\C}}\rmod \mu_3$ & $\mu_3$ & $S_2\times S_2$ \\ \hline \hline
		$A_1\times A_1$ & ? & ? & ? \\ \hline
		$G_2\times A_1$ & ? & ? & ? \\ \hline \hline
		$A_1\times A_3\times A_3$ & $\coset{\bk{\bk{SL_4\bk{\C}\rmod \mu_2}^2\rmod \mu_2}\times SL_2\bk{\C}}\rmod \mu_2$ & $\mu_2$ & $S_2^3$ \\ \hline
		$E_6\times A_2$ & $\bk{E_6^{sc}\times SL_3\bk{\C}} \rmod \mu_3$ & $\mu_3$ & $S_2^2$ \\ \hline
		$A_7\times A_1$ & $\bk{SL_8\bk{\C}\rmod \mu_2} \times PGL_2\bk{\C}$ & $\mu_4$ & $S_2$ \\ \hline
		$D_5\times A_3$ & $\bk{Spin_{10}\bk{\C} \times SL_4\bk{\C}} \rmod \mu_4$ & $\mu_4$ & $S_2^2$ \\ \hline
	\end{longtable}
	\label{Table:E7_proper_maximal_cuspidal_endoscopic_groups}
\end{center}

In the following table, we sort data on square-integrable residues $\ResRep{G}{i}{s_0}{\chi}$, with non-trivial $\chi$, as in the $E_6$ case.

%\begin{center}
%	\begin{longtable}[h]{|c|c|c|c|c|}
%		\hline
%		Orbit & $\sigma_{\psi_v}$ & $\bk{i,s_0,ord\bk{\chi}}$ & $Type\bk{\check{H}}$ & $S_\psi$
%		\\ \hline \endhead \hline
%		$E_7\bk{a_3}$ & $\esevenchar{1}{\chi}{\chi}{1}{\chi}{1}{1}$ & $\bk{1,\frac12,2}$, $\bk{3,\frac52,2}$, $\bk{4,2,2}$, $\bk{6,\frac52,2}$ & $D_6\times A_1$ & ? \\ \hline
%		$E_7\bk{a_4}$ & $\esevenchar{1}{\chi}{\chi}{1}{\chi}{\chi}{1}$ & $\bk{3,\frac32,2}$, $\bk{6,\frac12,2}$ & $G_2\times A_1$ & ? \\ \hline
%		$E_7\bk{a_5}$ &  $\esevenchar{\chi}{\chi}{\chi}{1}{\chi}{\chi}{1}$ & $\bk{3,\frac12,2}$, $\bk{4,1,2}$ & $A_1\times A_1$ & ? \\
%		& & $\bk{3,\frac12,3}$, $\bk{4,1,3}$, $\bk{5,1,3}$ & $A_5\times A_2$ & ? \\ \hline
%%		$E_7\bk{a_5}$ &  $\esevenchar{\chi}{\chi}{\chi}{1}{\chi}{\chi}{1}$ & $\bk{3,\frac12,3}$, $\bk{4,1,3}$, $\bk{5,1,3}$ & $A_5\times A_2$ & ? \\ \hline
%		$E_6\bk{a_1}$ & $\esevenchar{1}{\chi}{\chi}{1}{\chi}{1}{\chi}$ & $\bk{2,2,2}$, $\bk{5,2,2}$ & $A_7$ & ? \\ \hline
%		$A_4+A_1$ & $\esevenchar{\frac12+\chi}{\chi^2}{\chi^2}{\frac12+\chi}{\chi^2}{\frac12+\chi}{\chi^2}$ & $\bk{4,\frac12,4}$ & ? & ? \\ \hline %%% Type of Hv is A1, then we get the principal orbit.
%	\end{longtable}
%	\label{Table:E7_Arthur_Chi_Non-trivial}
%\end{center}

\begin{center}
	\begin{longtable}[h]{|c|c|c|c|}
		\hline
		Orbit & $\sigma_{\psi_v}$ & $\bk{i,s_0,ord\bk{\chi}}$ & $Type\bk{\check{H}}$ 
		\\ \hline \endhead \hline
		$E_7\bk{a_3}$ & $\esevenchar{1}{\chi}{\chi}{1}{\chi}{1}{1}$ & $\bk{1,\frac12,2}$, $\bk{3,\frac52,2}$, $\bk{4,2,2}$, $\bk{6,\frac52,2}$ & $D_6\times A_1$  \\ \hline
		$E_7\bk{a_4}$ & $\esevenchar{1}{\chi}{\chi}{1}{\chi}{\chi}{1}$ & $\bk{3,\frac32,2}$, $\bk{6,\frac12,2}$ & $D_6\times A_1$ \\ \hline % $D_6\bk{a_1}\times A_1$ $G_2\times A_1$
		$E_7\bk{a_5}$ &  $\esevenchar{\chi}{\chi}{\chi}{1}{\chi}{\chi}{1}$ & $\bk{3,\frac12,2}$, $\bk{4,1,2}$ & $D_6\times A_1$ \\ %$D_6\bk{a_2}\times A_1$
		& & $\bk{3,\frac12,3}$, $\bk{4,1,3}$, $\bk{5,1,3}$ & $A_5\times A_2$ \\ \hline
		%		$E_7\bk{a_5}$ &  $\esevenchar{\chi}{\chi}{\chi}{1}{\chi}{\chi}{1}$ & $\bk{3,\frac12,3}$, $\bk{4,1,3}$, $\bk{5,1,3}$ & $A_5\times A_2$ & ? \\ \hline
		$E_6\bk{a_1}$ & $\esevenchar{1}{\chi}{\chi}{1}{\chi}{1}{\chi}$ & $\bk{2,2,2}$, $\bk{5,2,2}$ & $A_7$ \\ \hline
		$A_4+A_1$ & $\esevenchar{\frac12+\chi}{\chi^2}{\chi^2}{\frac12+\chi}{\chi^2}{\frac12+\chi}{\chi^2}$ & $\bk{4,\frac12,4}$ & $A_1\times A_3\times A_3$ \\ \hline %%% Type of Hv is A1, then we get the principal orbit.
	\end{longtable}
	\label{Table:E7_Arthur_Chi_Non-trivial}
\end{center}

\sepline

For the orbits $E_7\bk{a_3}$,... and ...
a similar analysis to that of the orbit $E_6\bk{a_3}$ is valid. 

\begin{itemize}
	\item $E_6\bk{a_1}$ is not distinguished but it is quasi-distinguished, even and special.
	The parameter factors through $D_6\times A_1$, where $\phi$ corresponds to the orbit $D_6\bk{a_1}\times A_1$.
%	\item $E_6\bk{a_1}$ could possibly factor through the copy of $A_2$ as in Lawther (table 33).
	\item $A_4+A_1$ is not distinguished or even but it is quasi-distinguished and special.
%	The parameter factors through a copy of $A_1$ within the copy stated in Lawther-Testerman. This should be an $A_1$ maximal subgroup of the $A_2$ above.
	
	\redcolor{But how a character of order $4$ can arise this way?!?}
\end{itemize}




%\begin{center}
%	\begin{longtable}[h]{|c|c|c|c|}
%		\hline
%		Orbit & $\Real\bk{\lambda_{dom.}}$ & $\bk{i,s_0}$ & Comp 
%%		& $\Card{Sp\bk{\mO}}$
%		\\ \hline \endhead \hline
%		$E_7\bk{a_3}$ & $\esevenchar{1}{0}{0}{1}{0}{1}{1}$
%		& $\bk{1,\frac12,2}$, $\bk{3,\frac52,2}$, $\bk{4,2,2}$, $\bk{6,\frac52,2}$ & $S_2$ \\ \hline
%%		& 2 \\ \hline
%		$E_7\bk{a_4}$ & $\esevenchar{1}{0}{0}{1}{0}{0}{1}$
%		& $\bk{3,\frac32,2}$, $\bk{6,\frac12,2}$ & $S_2$ \\ \hline
%%		& 2 \\ \hline
%		$E_7\bk{a_5}$ &  $\esevenchar{0}{0}{0}{1}{0}{0}{1}$
%		& \begin{tabular}{c}
%			$\bk{3,\frac12,2}$, $\bk{4,1,2}$ \\ $\bk{3,\frac12,3}$, $\bk{4,1,3}$, $\bk{5,1,3}$
%		\end{tabular} & $S_3$ \\ \hline
%%		& 3 \\ \hline
%		$E_6\bk{a_1}$ & $\esevenchar{1}{0}{0}{1}{0}{1}{0}$ & $\bk{2,2,2}$, $\bk{5,2,2}$ & $S_2$ \\ \hline
%%		& 2 \\ \hline
%		$A_4+A_1$ & $\esevenchar{\frac12}{0}{0}{\frac12}{0}{\frac12}{0}$ & $\bk{4,\frac12,4}$ & $S_2$ \\ \hline
%%		& 2 \\ \hline
%	\end{longtable}
%%	\label{Table:E7_Arthur_Chi_Non-trivial}
%\end{center}
%
%\begin{itemize}
%	\item $E_6\bk{a_1}$ is not distinguished but it is quasi-distinguished, even and special.
%	\item $A_4+A_1$ is not distinguished or even but it is quasi-distinguished and special.
%	\item The following pairs are in the same orbit:
%	\begin{itemize}
%		\item $\bk{3,\frac12,2}$ and $\bk{4,1,2}$.
%		\item $\bk{3,\frac32,2}$ and $\bk{6,\frac12,2}$.
%	\end{itemize}
%\end{itemize}
%
%\begin{center}
%	\begin{longtable}[h]{|c|c|c|}
%		\hline
%		Orbit &  $\Real\bk{\lambda_{dom.}}$ & $\mu\bk{Fr_v}$ \\ \hline \endhead \hline
%		$E_7\bk{a_3}$ & $\esevenchar{1}{0}{0}{1}{0}{1}{1}$
%		& $\esevenchar{0}{\chi}{\chi}{0}{\chi}{0}{0}$ \\ \hline
%		$E_7\bk{a_4}$ & $\esevenchar{1}{0}{0}{1}{0}{0}{1}$
%		& $\esevenchar{0}{\chi}{\chi}{0}{\chi}{\chi}{0}$ \\ \hline
%		$E_7\bk{a_5}$ &  $\esevenchar{0}{0}{0}{1}{0}{0}{1}$
%		& $\esevenchar{\chi}{\chi}{\chi}{0}{\chi}{\chi}{0}$ \\ \hline
%		$E_6\bk{a_1}$ & $\esevenchar{1}{0}{0}{1}{0}{1}{0}$ & $\esevenchar{0}{\chi}{\chi}{0}{\chi}{0}{\chi}$ \\ \hline
%		$A_4+A_1$ & $\esevenchar{\frac12}{0}{0}{\frac12}{0}{\frac12}{0}$ & $\esevenchar{\chi}{\chi^2}{\chi^2}{\chi}{\chi^2}{\chi}{\chi^2}$ {\color{red}$\ast$} \\ \hline
%	\end{longtable}
%	\label{Table:E7_Arthur_Chi_Non-trivial_dom}
%\end{center}

\begin{center}
	\begin{longtable}[h]{|c|c|c|c|}
%	\begin{longtable}[H]{|c|c|c|c|}
		\hline
		$C_G$ & $H$ & $C_H$ & Principal
		%		& $\Card{Sp\bk{\mO}}$
		\\ \hline \endhead \hline
		$E_7\bk{a_3}$ & $D_6\times A_1$ & $D_6\oplus A_1$ & \cmark \\ \hline
		$E_7\bk{a_4}$ & $D_6\times A_1$ & $D_6\bk{a_1}\oplus A_1$ & \xmark \\
		 & $G_2\times A_1$ & $G_2\oplus A_1$ & \cmark \\ \hline
		$E_7\bk{a_5}$ & $D_6\times A_1$ & $D_6\bk{a_2}\oplus A_1$ & \xmark \\
		& $A_5\times A_2$ & $A_5\oplus A_2$ & \cmark \\
		 & $A_1\times A_1$ & $A_1\oplus A_1$ & \cmark \\ \hline
		$E_6\bk{a_1}$ & $A_7$ & $A_7$ & \cmark \\ 
		& $A_2$ & $A_2$ & \cmark \\ \hline
		$A_4+A_1$ & $A_2$ & $A_1$ & \xmark \\ \hline
	\end{longtable}
	\label{Table:E7_Orbits_and_Endoscopy}
\end{center}

%\redcolor{Note that $G_2\times A_1$ is a subgroup of $E_8$ which does not contain a maximal torus.}


\subsection{Case of $E_8$}

The extended Dynkin diagram of type $E_7$ is 
\[\begin{tikzpicture}[scale=0.5]
	\draw (-1,0) node[anchor=east]{};
	\draw (0 cm,0) -- (14 cm,0);
	\draw (4 cm, 0 cm) -- +(0,2 cm);
	\draw[fill=black] (0 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_1$};
	\draw[fill=black] (2 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_3$};
	\draw[fill=black] (4 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_4$};
	\draw[fill=black] (6 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_5$};
	\draw[fill=black] (8 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_6$};
	\draw[fill=black] (10 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_7$};
	\draw[fill=black] (12 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_8$};
	\draw[fill=black] (4 cm, 2 cm) circle (.25cm) node[right=3pt]{$\alpha_2$};
	\draw[fill=black] (14 cm, 0 cm) circle (.25cm) node[below=4pt]{$\alpha_0$};
\end{tikzpicture}\]

The proper maximal cuspidal endoscopic groups $H$ of $E_8$ have a complex dual $\check{H}$ of type
$D_8$, $A_8$, $A_4\times A_4$, $E_6\times A_2$ and $E_7\times A_1$, these can be attained by removing the roots $\alpha_1$, $\alpha_2$, $\alpha_5$, $\alpha_7$ and $\alpha_8$ (repectively) from the extended Dynkin diagram.
The group $E_8$ also admits endoscopic groups $H$ with $\check{H}$ of type $F_4\times G_2$, $B_2$ and $A_2\times A_1$, these are maximal among subgroups not containing a maximal torus.

\begin{center}
	\begin{longtable}[h]{|c|c|c|c|}
		\hline
		$Type\bk{\check{H}}$ & $\check{H}$ & $\cZ\bk{\check{H}}$ & $Out\bk{\check{H}}$
		\\ \hline \endhead \hline
		$D_8$ & $Spin_{16}\bk{\C}\rmod \mu_2$ & $\mu_2$ & $S_2$ \\ \hline
		$A_8$ & $SL_9\bk{\C}\rmod\mu_3$ & $\mu_3$ & $S_2$ \\ \hline
		$A_4\times A_4$ & $SL_5\bk{\C}\times PGL_5\bk{\C}$ & $\mu_5$ & $S_2\times S_2$ \\ \hline
		$E_6\times A_2$ & $\bk{E_6^{sc}\bk{\C}\times SL_3\bk{\C}} \rmod \mu_3$ & $\mu_3$ & $S_2\times S_2$ \\ \hline
		$E_7\times A_1$ & $\bk{E_7^{sc}\bk{\C}\times SL_2\bk{\C}}\rmod \mu_2$ & $\mu_2$ & $1$ \\ \hline \hline
		$F_4\times G_2$ &&& \\ \hline
		$B_2$ &&& \\ \hline
		$A_2\times A_1$ &&& \\ \hline \hline
		$D_5\times A_3$ & $\bk{Spin_{10}\bk{\C} \times SL_4\bk{\C}}\rmod \mu_4$ & $\mu_4$ & $S_2$ \\ \hline
		$A_5\times A_2 \times A_1$ & $\bk{ SL_6\bk{\C} \times SL_3\bk{\C} \times SL_2\bk{\C} } \rmod \mu_6$ & $\mu_6$ & $1$\\ \hline
	\end{longtable}
	\label{Table:E8_proper_maximal_cuspidal_endoscopic_groups}
\end{center}

In the following table, we sort data on square-integrable residues $\ResRep{G}{i}{s_0}{\chi}$, with non-trivial $\chi$, as in the $E_6$ case.

%\begin{center}
%	\begin{longtable}[h]{|c|c|c|c|c|}
%		\hline
%		Orbit & $\sigma_{\psi_v}$ & $\bk{i,s_0,ord\bk{\chi}}$ & $Type\bk{\check{H}}$ & $S_\psi$
%		\\ \hline \endhead \hline
%		$E_8\bk{a_3}$ & $\eeightchar{1}{\chi}{\chi}{1}{\chi}{1}{1}{1}$ & $\bk{3,\frac72,2}$, $\bk{4,\frac52,2}$, $\bk{7,\frac92,2}$, $\bk{8,\frac12,2}$ & $E_7\times A_1$ & ? \\ \hline
%		$E_8\bk{a_4}$ & $\eeightchar{1}{\chi}{\chi}{1}{\chi}{1}{\chi}{1}$ & $\bk{1,\frac72,2}$, $\bk{2,\frac72,2}$, $\bk{5,\frac52,2}$, $\bk{6,3,2}$ & $D_8$ & ? \\ \hline
%		$E_8\bk{b_4}$ & $\eeightchar{1}{\chi}{\chi}{1}{\chi}{\chi}{1}{1}$ & $\bk{3,\frac52,2}$, $\bk{7,\frac52,2}$ &?&?\\ \hline
%		$E_8\bk{a_5}$ & $\eeightchar{1}{\chi}{\chi}{1}{\chi}{\chi}{1}{\chi}$ & $\bk{1,\frac12,2}$, $\bk{2,\frac52,2}$ & $F_4\times G_2$ & ? \\ \hline
%		$E_8\bk{b_5}$ & $\eeightchar{\chi}{\chi}{\chi}{1}{\chi}{\chi}{1}{1}$ & $\bk{4,\frac32,2}$, $\bk{7,\frac12,2}$ &?&? \\
%		&& $\bk{4,\frac32,3}$, $\bk{6,2,3}$, $\bk{7,\frac12,3}$ & $E_6\times A_2$? & ? \\ \hline
%		$E_8\bk{a_6}$ & $\eeightchar{\chi}{\chi}{\chi}{1}{\chi}{\chi}{1}{\chi}$ & $\bk{2,\frac32,2}$, $\bk{5,\frac32,2}$ & $B_2$ & ? \\
%		&& $\bk{2,\frac32,3}$, $\bk{3,\frac32,3}$, $\bk{5,\frac32,3}$ & $A_8$ & ? \\ \hline
%		$E_8\bk{b_6}$ & $\eeightchar{\chi}{\chi}{\chi}{1}{\chi}{\chi}{\chi}{1}$ & $\bk{2,\frac12,2}$, $\bk{6,1,2}$ & ? &? \\
%		&& $\bk{6,1,3}$ \\ \hline
%		$E_8\bk{a_7}$ &  $\eeightchar{\chi}{\chi}{\chi}{\chi}{1}{\chi}{\chi}{\chi}$ & $\bk{5,\frac12,2}$ & $A_2\times A_1$? & ? \\
%		&& $\bk{4,\frac12,3}$ & $A_2\times A_1$? & ? \\
%		&& $\bk{5,\frac12,4}$ &?&? \\
%		&& $\bk{4,\frac12,5}$, $\bk{5,\frac12,5}$ & $A_4\times A_4$ & ? \\
%		& $\eeightchar{\chi^2}{\chi^2}{\chi^2}{\chi^3}{1}{\chi^3}{\chi^2}{\chi^2}$ & $\bk{4,\frac12,6}$ & $A_2\times A_1$? & ? \\ \hline
%		$D_5+A_2$ & $\eeightchar{\chi}{\chi}{\chi}{\chi}{1}{\chi}{\chi}{1}$ & $\bk{3,\frac12,2}$ &?&? \\ \hline
%		$E_6\bk{a_1}+A_1$ & $\eeightchar{\frac12+\chi}{\chi^2}{\chi^2}{\frac12+\chi}{\chi^2}{\frac12+\chi}{\chi^2}{1}$ & $\bk{3,1,4}$, $\bk{4,1,4}$ &?&? \\ \hline
%		$D_7\bk{a_2}$ & $\eeightchar{\frac12}{\chi}{\chi}{\frac12}{\chi}{\frac12}{\chi}{\frac12}$ & $\bk{5,1,2}$, $\bk{6,\frac12,2}$ &?&? \\
%		& $\eeightchar{\frac12+\chi}{\chi^2}{\chi^2}{\frac12+\chi}{\chi^2}{\frac12+\chi}{\chi^2}{\frac12+\chi}$  &  $\bk{5,1,4}$, $\bk{6,\frac12,4}$ &?&?  \\ \hline
%	\end{longtable}
%	\label{Table:E8_Arthur_Chi_Non-trivial}
%\end{center}

\begin{center}
	\begin{longtable}[h]{|c|c|c|c|}
		\hline
		Orbit & $\sigma_{\psi_v}$ & $\bk{i,s_0,ord\bk{\chi}}$ & $Type\bk{\check{H}}$
		\\ \hline \endhead \hline
		$E_8\bk{a_3}$ & $\eeightchar{1}{\chi}{\chi}{1}{\chi}{1}{1}{1}$ & $\bk{3,\frac72,2}$, $\bk{4,\frac52,2}$, $\bk{7,\frac92,2}$, $\bk{8,\frac12,2}$ & $E_7\times A_1$ \\ \hline
		$E_8\bk{a_4}$ & $\eeightchar{1}{\chi}{\chi}{1}{\chi}{1}{\chi}{1}$ & $\bk{1,\frac72,2}$, $\bk{2,\frac72,2}$, $\bk{5,\frac52,2}$, $\bk{6,3,2}$ & $D_8$ \\ \hline
		$E_8\bk{b_4}$ & $\eeightchar{1}{\chi}{\chi}{1}{\chi}{\chi}{1}{1}$ & $\bk{3,\frac52,2}$, $\bk{7,\frac52,2}$ &? \\ \hline
		$E_8\bk{a_5}$ & $\eeightchar{1}{\chi}{\chi}{1}{\chi}{\chi}{1}{\chi}$ & $\bk{1,\frac12,2}$, $\bk{2,\frac52,2}$ & ? \\ \hline
		$E_8\bk{b_5}$ & $\eeightchar{\chi}{\chi}{\chi}{1}{\chi}{\chi}{1}{1}$ & $\bk{4,\frac32,2}$, $\bk{7,\frac12,2}$ &? \\
		&& $\bk{4,\frac32,3}$, $\bk{6,2,3}$, $\bk{7,\frac12,3}$ & $E_6\times A_2$ \\ \hline
		$E_8\bk{a_6}$ & $\eeightchar{\chi}{\chi}{\chi}{1}{\chi}{\chi}{1}{\chi}$ & $\bk{2,\frac32,2}$, $\bk{5,\frac32,2}$ & ? \\
		&& $\bk{2,\frac32,3}$, $\bk{3,\frac32,3}$, $\bk{5,\frac32,3}$ & $A_8$ \\ \hline
		$E_8\bk{b_6}$ & $\eeightchar{\chi}{\chi}{\chi}{1}{\chi}{\chi}{\chi}{1}$ & $\bk{2,\frac12,2}$, $\bk{6,1,2}$ & ? \\
		&& $\bk{6,1,3}$ & \\ \hline
		$E_8\bk{a_7}$ &  $\eeightchar{\chi}{\chi}{\chi}{\chi}{1}{\chi}{\chi}{\chi}$ & $\bk{5,\frac12,2}$ & $A_5\times A_2 \times A_1$  \\
		&& $\bk{4,\frac12,3}$ & $A_5\times A_2 \times A_1$ \\
		&& $\bk{5,\frac12,4}$ & $D_5\times A_3$ \\
		&& $\bk{4,\frac12,5}$, $\bk{5,\frac12,5}$ & $A_4\times A_4$ \\
		& $\eeightchar{\chi^2}{\chi^2}{\chi^2}{\chi^3}{1}{\chi^3}{\chi^2}{\chi^2}$ & $\bk{4,\frac12,6}$ & $A_5\times A_2 \times A_1$ \\ \hline
		$D_5+A_2$ & $\eeightchar{\chi}{\chi}{\chi}{\chi}{1}{\chi}{\chi}{1}$ & $\bk{3,\frac12,2}$ &? \\ \hline
		$E_6\bk{a_1}+A_1$ & $\eeightchar{\frac12+\chi}{\chi^2}{\chi^2}{\frac12+\chi}{\chi^2}{\frac12+\chi}{\chi^2}{1}$ & $\bk{3,1,4}$, $\bk{4,1,4}$ &? \\ \hline
		$D_7\bk{a_2}$ & $\eeightchar{\frac12}{\chi}{\chi}{\frac12}{\chi}{\frac12}{\chi}{\frac12}$ & $\bk{5,1,2}$, $\bk{6,\frac12,2}$ &? \\
		& $\eeightchar{\frac12+\chi}{\chi^2}{\chi^2}{\frac12+\chi}{\chi^2}{\frac12+\chi}{\chi^2}{\frac12+\chi}$  &  $\bk{5,1,4}$, $\bk{6,\frac12,4}$ &?  \\ \hline
	\end{longtable}
	\label{Table:E8_Arthur_Chi_Non-trivial}
\end{center}

\todonum{Check the imaginary parts}

\begin{itemize}
	\item In the case of the orbit $E_8\bk{a_7}$ with characters of order $2$, $3$ and $6$, we factor the parameter through the same pseudo-Levi subgroup and the order of $\chi$ depends on the order of the image of $W_F$ in the center of $\check{H}$.
	
	In the case of $\chi$ of order $4$, the parameter factors through $D_5\times A_3$ and $\phi$ corresponds to the orbit $D_5\bk{a_1}+A_3$.
	
	\item $D_5+A_2$ is not distinguished but it is quasi-distinguished, even and special.
	\item $E_6\bk{a_1}+A_1$ and $D_7\bk{a_2}$ are not distinguished or even but are quasi-distinguished and special.
	\item $D_7\bk{a_1}$ is also quasi-distinguished, but seems like there is not degenerate principal series representation with a suitable anti-dominant exponent.
\end{itemize}
\todonum{Is $\bk{6,\frac12,2}$ square integrable? It should be according to the table.}

\sepline

%\begin{center}
%	\begin{longtable}[h]{|c|c|c|c|}
	%	\begin{longtable}[H]{|c|c|c|c|}
%		\hline
%		Orbit & $\Real\bk{\lambda_{dom.}}$ & $\bk{i,s_0}$ & Comp 
%%			& $\Card{Sp\bk{\mO}}$
%		\\ \hline \endhead \hline
%		$E_8\bk{a_3}$ & $\eeightchar{1}{0}{0}{1}{0}{1}{1}{1}$ &
%		$\bk{3,\frac72,2}$, $\bk{4,\frac52,2}$, $\bk{7,\frac92,2}$, $\bk{8,\frac12,2}$
%		& $S_2$ \\ \hline
%%			& 2 \\ \hline
%		$E_8\bk{a_4}$ & $\eeightchar{1}{0}{0}{1}{0}{1}{0}{1}$ &
%		$\bk{1,\frac72,2}$, $\bk{2,\frac72,2}$, $\bk{5,\frac52,2}$, $\bk{6,3,2}$
%		& $S_2$ \\ \hline
%			& 2 \\ \hline
%		$E_8\bk{b_4}$ & $\eeightchar{1}{0}{0}{1}{0}{0}{1}{1}$ & 
%		$\bk{3,\frac52,2}$, $\bk{7,\frac52,2}$
%		& $S_2$ \\ \hline
%%			& 2 \\ \hline
%		$E_8\bk{a_5}$ & $\eeightchar{1}{0}{0}{1}{0}{0}{1}{0}$ & 
%		$\bk{1,\frac12,2}$, $\bk{2,\frac52,2}$
%		& $S_2$ \\ \hline
%%			& 2 \\ \hline
%		$E_8\bk{b_5}$ & $\eeightchar{0}{0}{0}{1}{0}{0}{1}{1}$ & 
%		\begin{tabular}{c}
%			$\bk{4,\frac32,2}$, $\bk{7,\frac12,2}$ \\ $\bk{4,\frac32,3}$, $\bk{6,2,3}$, $\bk{7,\frac12,3}$
%		\end{tabular}
%		& $S_3$ \\ \hline
%%			& 3 \\ \hline
%		$E_8\bk{a_6}$ & $\eeightchar{0}{0}{0}{1}{0}{0}{1}{0}$ & 
%		\begin{tabular}{c}
%			$\bk{2,\frac32,2}$, $\bk{5,\frac32,2}$\\
%			$\bk{2,\frac32,3}$, $\bk{3,\frac32,3}$, $\bk{5,\frac32,3}$
%		\end{tabular} & $S_3$ \\ \hline
%%			& 3 \\ \hline
%		$E_8\bk{b_6}$ & $\eeightchar{0}{0}{0}{1}{0}{0}{0}{1}$ & 
%		\begin{tabular}{c}
%			$\bk{2,\frac12,2}$, $\bk{6,1,2}$ \\
%			$\bk{6,1,3}$
%		\end{tabular} & $S_3$ \\ \hline
%%			& 3 \\ \hline
%		$E_8\bk{a_7}$ & $\eeightchar{0}{0}{0}{0}{1}{0}{0}{0}$ & 
%		\begin{tabular}{c}
%			$\bk{5,\frac12,2}$ \\
%			$\bk{4,\frac12,3}$ \\
%			$\bk{5,\frac12,4}$ \\
%			$\bk{4,\frac12,5}$, $\bk{5,\frac12,5}$ \\
%			$\bk{4,\frac12,6}$
%		\end{tabular} & $S_5$ \\ \hline
%%			& 6 \\ \hline
%		$D_5+A_2$ & $\eeightchar{0}{0}{0}{0}{1}{0}{0}{1}$ & 
%		$\bk{3,\frac12,2}$
%		& $S_2$ \\ \hline
%%			& 2 \\ \hline
%		$E_6\bk{a_1}+A_1$ & $\eeightchar{\frac12}{0}{0}{\frac12}{0}{\frac12}{0}{1}$ & 
%		$\bk{3,1,4}$, $\bk{4,1,4}$
%		& $S_2$ \\ \hline
%%			& 2 \\ \hline
%		$D_7\bk{a_2}$ & $\eeightchar{\frac12}{0}{0}{\frac12}{0}{\frac12}{0}{\frac12}$ & 
%		\begin{tabular}{c}
%			$\bk{5,1,2}$, $\bk{6,\frac12,2}$ \\ $\bk{5,1,4}$, $\bk{6,\frac12,4}$
%		\end{tabular}
%		& $S_2$ \\ \hline
%%			& 2 \\ \hline
%	\end{longtable}
%%	\label{Table:E8_Arthur_Chi_Non-trivial}
%\end{center}


%$\lambda_{dom.} = \psi\bk{Fr_v,\begin{pmatrix}q^{\frac12} & \\ & 1^{-\frac12} \end{pmatrix}}$
%
%\begin{center}
%	\begin{longtable}[h]{|c|c|}
%		%	\begin{longtable}[H]{|c|c|c|c|}
%			\hline
%			Orbit & $\lambda_{dom.}$ \\ \hline \endhead \hline
%			$E_8\bk{a_3}$ & $\eeightchar{1}{\chi}{\chi}{1}{\chi}{1}{1}{1}$ \\ \hline
%			$E_8\bk{a_4}$ & $\eeightchar{1}{\chi}{\chi}{1}{\chi}{1}{\chi}{1}$ \\ \hline
%			$E_8\bk{b_4}$ & $\eeightchar{1}{\chi}{\chi}{1}{\chi}{\chi}{1}{1}$ \\ \hline
%			$E_8\bk{a_5}$ & $\eeightchar{1}{\chi}{\chi}{1}{\chi}{\chi}{1}{\chi}$ \\ \hline
%			$E_8\bk{b_5}$ & $\eeightchar{\chi}{\chi}{\chi}{1}{\chi}{\chi}{1}{1}$ \\ \hline
%			$E_8\bk{a_6}$ & $\eeightchar{\chi}{\chi}{\chi}{1}{\chi}{\chi}{1}{\chi}$ \\ \hline
%			$E_8\bk{b_6}$ & $\eeightchar{\chi}{\chi}{\chi}{1}{\chi}{\chi}{\chi}{1}$ \\ \hline
%			$E_8\bk{a_7}$ &  
%			\begin{tabular}{cc}
%				$\eeightchar{\chi}{\chi}{\chi}{\chi}{1}{\chi}{\chi}{\chi}$ & $ord\bk{\chi}=2,3,4,5$ \\ & \\
%				$\eeightchar{\chi^2}{\chi^2}{\chi^2}{\chi^3}{1}{\chi^3}{\chi^2}{\chi^2}$ & $ord\bk{\chi}=6$ {\color{red}$\ast$}
%			\end{tabular} \\ \hline
%			$D_5+A_2$ & $\eeightchar{\chi}{\chi}{\chi}{\chi}{1}{\chi}{\chi}{1}$ \\ \hline
%			$E_6\bk{a_1}+A_1$ & $\eeightchar{\frac12+\chi^3}{\chi^2}{\chi^2}{\frac12+\chi^3}{\chi^2}{\frac12+\chi^3}{\chi^2}{1+\chi^2}$ {\color{red}$\ast$} \\ \hline
%			$D_7\bk{a_2}$ &
%			\begin{tabular}{cc}
%				$\eeightchar{\frac12}{\chi}{\chi}{\frac12}{\chi}{\frac12}{\chi}{\frac12}$ & $ord\bk{\chi}=2$ \\ & \\
%				$\eeightchar{\frac12+\chi}{\chi^2}{\chi^2}{\frac12+\chi^3}{\chi^2}{\frac12+\chi^3}{\chi^2}{\frac12+\chi^3}$  & $ord\bk{\chi}=4$ {\color{red}$\ast$}
%			\end{tabular} \\ \hline
%		\end{longtable}
%		\label{Table:E8_Arthur_Chi_Non-trivial_dom}
%	\end{center}


%\begin{itemize}
%	\item $D_5+A_2$ is not distinguished but it is quasi-distinguished, even and special.
%	\item $E_6\bk{a_1}+A_1$ and $D_7\bk{a_2}$ are not distinguished or even but are quasi-distinguished and special.
%	\item $D_7\bk{a_1}$ is also quasi-distinguished, but seems like there is not degenerate principal series representation with a suitable anti-dominant exponent.
%	\item The following pairs are in the same orbit:
%	\begin{itemize}
%		\item $\bk{1,\frac12,2}$ and $\bk{2,\frac52,2}$.
%		\item $\bk{2,\frac12,2}$ and $\bk{6,1,2}$.
%		\item $\bk{2,\frac32,2}$ and $\bk{5,\frac32,2}$.
%		\item $\bk{3,\frac52,2}$ and $\bk{7,\frac52,2}$.
%		\item $\bk{4,\frac32,2}$ and $\bk{7,\frac12,2}$.
%	\end{itemize}
%\end{itemize}

\begin{center}
	\begin{longtable}[h]{|c|c|c|c|}
%	\begin{longtable}[H]{|c|c|c|c|}
		\hline
		$C_G$ & $H$ & $C_H$ & Principal
		%		& $\Card{Sp\bk{\mO}}$
		\\ \hline \endhead \hline
		$E_8\bk{a_3}$ & $E_7\times A_1$ & $E_7\oplus A_1$ & \cmark \\ \hline
		$E_8\bk{a_4}$ & $D_8$ & $D_8$ & \cmark \\ \hline
		$E_8\bk{b_4}$ & $E_7\times A_1$ & $E_7\bk{a_1}\oplus A_1$ & \xmark \\ \hline %%% It seems like $E_7\bk{a_1}$ is induced from the principal orbit of $A_1$.
		$E_8\bk{a_5}$ & $D_8$ & $D_8\bk{a_1}$ & \xmark \\
		& $F_4\times G_2$ & $F_4\oplus G_2$ & \cmark \\ \hline
		$E_8\bk{b_5}$ & $F_4\times G_2$ & $F_4\oplus G_2\bk{a_1}$ & \xmark\\
		& $E_7\times A_1$ & $E_7\bk{a_2}\oplus A_1$ & \xmark \\
		& $E_6\times A_2$ & $E_6\oplus A_2$ & \cmark \\ \hline
		$E_8\bk{a_6}$ & $D_8$ & $D_8\bk{a_2}$ & \xmark \\
		& $A_8$ & $A_8$ & \cmark \\ 
		 & $B_2$ & $B_2$ & \cmark \\ \hline
		$E_8\bk{b_6}$ & $D_8$ & $D_8\bk{a_3}$ & \xmark \\
		& $E_6\times A_2$ & $E_6\bk{a_1}\times A_2$ & \xmark \\
		& $F_4\times G_2$ & $F_4\bk{a_1}\oplus G_2$ & \xmark \\
		& $C_4\times A_2 \subset E_6\times A_2$ & $C_4\oplus A_2$ & \cmark \\ \hline
		$E_8\bk{a_7}$ & $D_8$ & $D_8\bk{a_5}$ & \xmark \\
		& $E_7\times A_1$ & $E_7\bk{a_5}\oplus A_1$ & \xmark \\
		& $E_6\times A_2$ & $E_6\bk{a_3}\oplus A_2$ & \xmark \\
		& $F_4\times G_2$ & $F_4\bk{a_2}\oplus G_2\bk{a_1}$ & \xmark \\
		& $A_4\times A_4$ & $A_4\oplus A_4$ & \cmark \\
		& $A_2\times A_1$ & $A_2\oplus A_1$ & \cmark \\ \hline
		$D_5+A_2$ & $E_7\times A_1$ & $E_7\bk{a_4}\oplus A_1$ & \xmark \\
		& $D_6\times A_1\times A_1$ & $D_6\bk{a_1}\oplus A_1\oplus A_1$ & \xmark \\
		& $F_4\times G_2$ & $F_4\bk{a_1}\oplus G_2\bk{a_1}$ & \xmark \\
		& $F_4\times G_2$ & $F_4\bk{a_2}\oplus G_2$ & \xmark \\ \hline %%% It seems like $F_4\bk{a_2}$ is induced from the principal orbit of $A_1\times A_{1,s}$.
		$E_6\bk{a_1}+A_1$ & ? & ? & ? \\ \hline %%% This might be induced from the principal orbit of $A_4\times A_1$ given by the simple roots $[1, 2, 3, 4, 6]$
		%%% Also, it meets the pseudolevi [[[0, 1, 2, 4, 5, 6, 7, 8], 4]]
		$D_7\bk{a_2}$ & ? & ? & ? \\ \hline %%% Could be connected to either of the following Levis [1, 2, 3, 4, 6, 8]	A4+2*A1, 	[1, 3, 4, 6, 7, 8]	2*A3
		%%% Also to the pseudo levi 	[[[0, 1, 2, 3, 4, 5, 7, 8], 4]]
	\end{longtable}
	\label{Table:E8_Orbits_and_Endoscopy}
\end{center}

%\redcolor{Note that $F_4\times G_2$ and $D_6\times A_1\times A_1$ and $C_4\times A_2$ are subgroups of $E_8$ which does not contain a maximal torus.}

